Feasibility of perturbative generation of bound-states from resonances or virtual states

I investigate whether it is possible to generate bound-states from resonances or virtual states through first-order perturbation theory. Using contact-type potentials as those appeared in pionless effective field theory, I show that it is possible to obtain negative-energy states by sandwiching a next-to-leading order (NLO) interaction with the leading-order (LO) wavefunctions, under the presence of LO resonances or virtual states. However, at least under the framework of time-independent Schr\"odinger equation and Hermitian Hamiltonian, there is an inability to create bound-states with structure similar to those formed by the non-perturbative treatments.

==> 1s0_nlo <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Fri Sep 10 13:13:05 2021"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.14, 250, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.157000, 0.550000, 1.260000, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label ""
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 50
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 0
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\SNLO\N\h{-1}\si\N   [MeV]"
@    yaxis  label layout para
@    yaxis  label place spec
@    yaxis  label place 0.000000, 0.120000
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.03
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.250000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.85, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  ""
@g1 on
@g1 hidden false
@g1 type XY
@g1 stacked false
@g1 bar hgap 0.000000
@g1 fixedpoint off
@g1 fixedpoint type 0
@g1 fixedpoint xy 0.000000, 0.000000
@g1 fixedpoint format general general
@g1 fixedpoint prec 6, 6
@with g1
@    world 0, 0.5, 250, 450
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.157000, 0.150000, 1.260000, 0.550000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "i\Sth"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 50
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\SLO\N\h{-1}\si\N   + E\SNLO\N\h{-1}\si\N   [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 100
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.250000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 0.250000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 1.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:2"
@    s0 legend  ""
@g2 on
@g2 hidden false
@g2 type XY
@g2 stacked false
@g2 bar hgap 0.000000
@g2 fixedpoint off
@g2 fixedpoint type 0
@g2 fixedpoint xy 0.000000, 0.000000
@g2 fixedpoint format general general
@g2 fixedpoint prec 6, 6
@with g2
@    world 0, -0.01, 4, 0.01
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.350000, 0.320000, 0.820000, 0.520000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "i\Sth"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 1
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\SLO\N\h{-1}\si\N  +E\SNLO\N\h{-1}\si\N   [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.005
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 1
@    s0 symbol size 0.500000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 2
@    s0 line linewidth 1.5
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/mares/jerry/test_per/fort.1556"
@    s0 legend  ""
@target G0.S0
@type xy
1 -0.0070945375
2 -0.02468691
3 -0.045599295
4 -0.064651544
5 -0.080058144
6 -0.091808402
7 -0.10067487
8 -0.10730177
9 -0.11236193
10 -0.11620882
11 -0.11923429
12 -0.12158265
13 -0.1234868
14 -0.1249882
15 -0.12623997
16 -0.12723511
17 -0.12808587
18 -0.12876196
19 -0.12935357
20 -0.1298188
21 -0.13023532
22 -0.13055518
23 -0.13084864
24 -0.13106442
25 -0.1312683
26 -0.13140697
27 -0.13154352
28 -0.13162327
29 -0.13170773
30 -0.13174114
31 -0.13178422
32 -0.13178023
33 -0.13178963
34 -0.13175471
35 -0.13173607
36 -0.131675
37 -0.13163254
38 -0.13154891
39 -0.13148582
40 -0.13138237
41 -0.13130113
42 -0.13117996
43 -0.13108248
44 -0.13094526
45 -0.13083306
46 -0.13068108
47 -0.13055537
48 -0.13038968
49 -0.13025145
50 -0.13007288
51 -0.1299229
52 -0.12973214
53 -0.12957108
54 -0.12936867
55 -0.12919705
56 -0.12898346
57 -0.12880172
58 -0.1285773
59 -0.12838581
60 -0.12815087
61 -0.12794993
62 -0.12770472
63 -0.12749458
64 -0.1272393
65 -0.12702016
66 -0.12675498
67 -0.12652701
68 -0.12625204
69 -0.12601539
70 -0.12573074
71 -0.12548551
72 -0.12519124
73 -0.12493751
74 -0.12463367
75 -0.1243715
76 -0.12405812
77 -0.12378755
78 -0.12346463
79 -0.12318568
80 -0.12285322
81 -0.12256588
82 -0.12222384
83 -0.1219281
84 -0.12157643
85 -0.12127227
86 -0.12091091
87 -0.12059827
88 -0.12022715
89 -0.11990596
90 -0.11952498
91 -0.11919518
92 -0.11880422
93 -0.11846571
94 -0.11806466
95 -0.11771732
96 -0.11730605
97 -0.11694976
98 -0.1165281
99 -0.11616274
100 -0.11573053
101 -0.11535593
102 -0.11491299
103 -0.11452899
104 -0.11407511
105 -0.11368153
106 -0.1132165
107 -0.11281314
108 -0.11233674
109 -0.11192339
110 -0.11143536
111 -0.11101179
112 -0.11051187
113 -0.11007784
114 -0.10956576
115 -0.109121
116 -0.10859647
117 -0.10814071
118 -0.10760342
119 -0.10713636
120 -0.10658597
121 -0.10610732
122 -0.10554349
123 -0.10505291
124 -0.10447528
125 -0.10397243
126 -0.10338062
127 -0.10286515
128 -0.10225877
129 -0.10173029
130 -0.10110893
131 -0.10056706
132 -0.099930278
133 -0.099374614
134 -0.098721973
135 -0.098152089
136 -0.09748313
137 -0.09689859
138 -0.096212837
139 -0.095613189
140 -0.094910155
141 -0.094294937
142 -0.09357412
143 -0.092942858
144 -0.092203746
145 -0.091555955
146 -0.090798028
147 -0.090133216
148 -0.089355947
149 -0.088673618
150 -0.087876475
151 -0.087176129
152 -0.086358583
153 -0.085639723
154 -0.084801244
155 -0.084063379
156 -0.083203449
157 -0.082446098
158 -0.081564213
159 -0.080786912
160 -0.079882588
161 -0.079084897
162 -0.078157678
163 -0.077339189
164 -0.076388657
165 -0.075549002
166 -0.074574787
167 -0.073713651
168 -0.072715442
169 -0.071832573
170 -0.07081013
171 -0.069905353
172 -0.068858527
173 -0.06793176
174 -0.066860504
175 -0.065911778
176 -0.064816171
177 -0.063845644
178 -0.062725909
179 -0.061733892
180 -0.060590421
181 -0.059577401
182 -0.058410779
183 -0.057377444
184 -0.056188479
185 -0.055135743
186 -0.053925494
187 -0.052854529
188 -0.051624336
189 -0.050536602
190 -0.049288118
191 -0.048185391
192 -0.046920613
193 -0.045805017
194 -0.044526318
195 -0.04340035
196 -0.042110506
197 -0.040977064
198 -0.039679279
199 -0.038541678
200 -0.0372396
201 -0.036101589
202 -0.034799322
203 -0.033665083
204 -0.032367187
205 -0.031241326
206 -0.029952798
207 -0.028840324
208 -0.027566573
209 -0.026472853
210 -0.025219642
211 -0.024150341
212 -0.022923722
213 -0.02188472
214 -0.020690935
215 -0.019688218
216 -0.018533585
217 -0.017573121
218 -0.01646389
219 -0.015551477
220 -0.014493672
221 -0.013634776
222 -0.01263402
223 -0.0118336
224 -0.010894933
225 -0.010157263
226 -0.0092849577
227 -0.0086134584
228 -0.0078108528
229 -0.0072079433
230 -0.0064772873
231 -0.0059442649
232 -0.0052866047
233 -0.0048235677
234 -0.0042386696
235 -0.003844493
236 -0.0033308136
237 -0.0030031861
238 -0.0025578914
239 -0.0022934213
240 -0.0019124458
241 -0.0017068487
242 -0.001384975
243 -0.0012333675
244 -0.0009642743
245 -0.00086166134
246 -0.00063779712
247 -0.00058008242
248 -0.00039184811
249 -0.00037920427
250 -0.00021045739
251 -0.00027784092
&
@target G1.S0
@type xy
1 -0.0029018358
2 -0.0077806891
3 -0.0071500725
4 0.0045017624
5 0.029197405
6 0.067126793
7 0.11759648
8 0.18005159
9 0.25382532
10 0.33862854
11 0.43404308
12 0.53998779
13 0.65618506
14 0.78266342
15 0.91921154
16 1.065916
17 1.2225948
18 1.3893686
19 1.5660665
20 1.752832
21 1.9494963
22 2.1562204
23 2.3728327
24 2.599509
25 2.8360721
26 3.0827112
27 3.3392419
28 3.6058665
29 3.8823919
30 4.1690332
31 4.4655882
32 4.7722845
33 5.0889103
34 5.4157057
35 5.7524488
36 6.0993925
37 6.4563045
38 6.8234505
39 7.2005875
40 7.5879942
41 7.9854166
42 8.3931464
43 8.8109189
44 9.2390387
45 9.6772299
46 10.12581
47 10.584493
48 11.05361
49 11.532861
50 12.022592
51 12.522493
52 13.032923
53 13.553558
54 14.084773
55 14.626233
56 15.178325
57 15.740703
58 16.313767
59 16.897161
60 17.491299
61 18.095812
62 18.711127
63 19.336865
64 19.973468
65 20.620544
66 21.278548
67 21.947077
68 22.626602
69 23.316706
70 24.017874
71 24.729679
72 25.452621
73 26.186258
74 26.931106
75 27.686713
76 28.453607
77 29.231324
78 30.020409
79 30.820385
80 31.631811
81 32.454198
82 33.288122
83 34.13308
84 34.989664
85 35.857358
86 36.736769
87 37.62737
88 38.529784
89 39.443471
90 40.369069
91 41.306026
92 42.254996
93 43.215414
94 44.187952
95 45.17203
96 46.168337
97 47.176282
98 48.196569
99 49.228594
100 50.273078
101 51.329405
102 52.398313
103 53.479172
104 54.572738
105 55.678369
106 56.796836
107 57.927485
108 59.071106
109 60.22703
110 61.396067
111 62.577534
112 63.772257
113 64.979544
114 66.200237
115 67.43363
116 68.680586
117 69.940384
118 71.213906
119 72.50042
120 73.800825
121 75.114375
122 76.441992
123 77.782914
124 79.138082
125 80.506724
126 81.8898
127 83.286523
128 84.697874
129 86.123055
130 87.563066
131 89.017096
132 90.486167
133 91.969453
134 93.467999
135 94.980967
136 96.509421
137 98.052512
138 99.611326
139 101.185
140 102.77465
141 104.37939
142 106.00036
143 107.63666
144 109.28947
145 110.95786
146 112.64304
147 114.34408
148 116.06218
149 117.79643
150 119.54805
151 121.31611
152 123.10185
153 124.90435
154 126.72487
155 128.56246
156 130.41842
157 132.29179
158 134.1839
159 136.09378
160 138.02277
161 139.96992
162 141.93658
163 143.92179
164 145.92695
165 147.95106
166 149.99556
167 152.05946
168 154.14423
169 156.24885
170 158.37484
171 160.52117
172 162.68939
173 164.87848
174 167.09001
175 169.32295
176 171.57892
177 173.8569
178 176.15852
179 178.48277
180 180.83132
181 183.20317
182 185.60002
183 188.02087
184 190.46747
185 192.93884
186 195.43674
187 197.96023
188 200.5111
189 203.08843
190 205.69406
191 208.32707
192 210.98938
193 213.68008
194 216.40113
195 219.15166
196 221.93369
197 224.74637
198 227.5918
199 230.46916
200 233.38061
201 236.32541
202 239.30575
203 242.32096
204 245.37333
205 248.46225
206 251.59009
207 254.75633
208 257.96344
209 261.21099
210 264.50155
211 267.83484
212 271.21355
213 274.63751
214 278.10957
215 281.62975
216 285.20105
217 288.82368
218 292.50086
219 296.23304
220 300.02367
221 303.87351
222 307.78629
223 311.76315
224 315.80817
225 319.92293
226 324.11199
227 328.37748
228 332.72454
229 337.15605
230 341.6779
231 346.2939
232 351.01099
233 355.83423
234 360.77197
235 365.83103
236 371.02175
237 376.35346
238 381.83947
239 387.49284
240 393.33152
241 399.37457
242 405.64763
243 412.1801
244 419.01175
245 426.19203
246 433.79034
247 441.90246
248 450.67581
249 460.35191
250 471.40012
251 485.03611
&
@target G2.S0
@type xy
0 -0.0029018358
1 -0.0077806891
2 -0.0071500725
3 0.0045017624
4 0.029197405
6 0.067126793
7 0.11759648
8 0.18005159
9 0.25382532
10 0.33862854
11 0.43404308
12 0.53998779
13 0.65618506
14 0.78266342
15 0.91921154
16 1.065916
17 1.2225948
18 1.3893686
19 1.5660665
20 1.752832
21 1.9494963
22 2.1562204
23 2.3728327
24 2.599509
25 2.8360721
26 3.0827112
27 3.3392419
28 3.6058665
29 3.8823919
30 4.1690332
31 4.4655882
32 4.7722845
33 5.0889103
34 5.4157057
35 5.7524488
36 6.0993925
37 6.4563045
38 6.8234505
39 7.2005875
40 7.5879942
41 7.9854166
42 8.3931464
43 8.8109189
44 9.2390387
45 9.6772299
46 10.12581
47 10.584493
48 11.05361
49 11.532861
50 12.022592
51 12.522493
52 13.032923
53 13.553558
54 14.084773
55 14.626233
56 15.178325
57 15.740703
58 16.313767
59 16.897161
60 17.491299
61 18.095812
62 18.711127
63 19.336865
64 19.973468
65 20.620544
66 21.278548
67 21.947077
68 22.626602
69 23.316706
70 24.017874
71 24.729679
72 25.452621
73 26.186258
74 26.931106
75 27.686713
76 28.453607
77 29.231324
78 30.020409
79 30.820385
80 31.631811
81 32.454198
82 33.288122
83 34.13308
84 34.989664
85 35.857358
86 36.736769
87 37.62737
88 38.529784
89 39.443471
90 40.369069
91 41.306026
92 42.254996
93 43.215414
94 44.187952
95 45.17203
96 46.168337
97 47.176282
98 48.196569
99 49.228594
100 50.273078
101 51.329405
102 52.398313
103 53.479172
104 54.572738
105 55.678369
106 56.796836
107 57.927485
108 59.071106
109 60.22703
110 61.396067
111 62.577534
112 63.772257
113 64.979544
114 66.200237
115 67.43363
116 68.680586
117 69.940384
118 71.213906
119 72.50042
120 73.800825
121 75.114375
122 76.441992
123 77.782914
124 79.138082
125 80.506724
126 81.8898
127 83.286523
128 84.697874
129 86.123055
130 87.563066
131 89.017096
132 90.486167
133 91.969453
134 93.467999
135 94.980967
136 96.509421
137 98.052512
138 99.611326
139 101.185
140 102.77465
141 104.37939
142 106.00036
143 107.63666
144 109.28947
145 110.95786
146 112.64304
147 114.34408
148 116.06218
149 117.79643
150 119.54805
151 121.31611
152 123.10185
153 124.90435
154 126.72487
155 128.56246
156 130.41842
157 132.29179
158 134.1839
159 136.09378
160 138.02277
161 139.96992
162 141.93658
163 143.92179
164 145.92695
165 147.95106
166 149.99556
167 152.05946
168 154.14423
169 156.24885
170 158.37484
171 160.52117
172 162.68939
173 164.87848
174 167.09001
175 169.32295
176 171.57892
177 173.8569
178 176.15852
179 178.48277
180 180.83132
181 183.20317
182 185.60002
183 188.02087
184 190.46747
185 192.93884
186 195.43674
187 197.96023
188 200.5111
189 203.08843
190 205.69406
191 208.32707
192 210.98938
193 213.68008
194 216.40113
195 219.15166
196 221.93369
197 224.74637
198 227.5918
199 230.46916
200 233.38061
201 236.32541
202 239.30575
203 242.32096
204 245.37333
205 248.46225
206 251.59009
207 254.75633
208 257.96344
209 261.21099
210 264.50155
211 267.83484
212 271.21355
213 274.63751
214 278.10957
215 281.62975
216 285.20105
217 288.82368
218 292.50086
219 296.23304
220 300.02367
221 303.87351
222 307.78629
223 311.76315
224 315.80817
225 319.92293
226 324.11199
227 328.37748
228 332.72454
229 337.15605
230 341.6779
231 346.2939
232 351.01099
233 355.83423
234 360.77197
235 365.83103
236 371.02175
237 376.35346
238 381.83947
239 387.49284
240 393.33152
241 399.37457
242 405.64763
243 412.1801
244 419.01175
245 426.19203
246 433.79034
247 441.90246
248 450.67581
249 460.35191
250 471.40012
251 485.03611
&


==> 1s0_phase <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Thu Sep  2 14:51:14 2021"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, 0, 270, 80
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 0.625703, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "T\slab\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 50
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\xd\0(\S1\NS\s0\N) [deg]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 10
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.85, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 2.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/mares/jerry/test_per/fort.76"
@    s1 legend  ""
@g1 on
@g1 hidden false
@g1 type XY
@g1 stacked false
@g1 bar hgap 0.000000
@g1 fixedpoint off
@g1 fixedpoint type 0
@g1 fixedpoint xy 0.000000, 0.000000
@g1 fixedpoint format general general
@g1 fixedpoint prec 6, 6
@with g1
@    world 0, 0, 3, 0.2
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.788414, 0.150000, 1.264118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "E\scm\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.5
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\xs\0(\S1\NS\s0\N) [MeV\S-2\N]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.05
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 2.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/mares/jerry/test_per/fort.708"
@    s1 legend  ""
@target G0.S1
@type xy
2.1300934e-05 0.69410921
8.5203735e-05 1.3880043
0.037574846 26.866886
0.14322747 44.334138
0.31704309 54.940811
0.55902169 61.499103
0.86916328 65.753837
1.2474679 68.635604
1.6939354 70.650459
2.208566 72.088515
2.7913595 73.125354
3.442316 73.872502
4.1614355 74.403796
4.948718 74.769873
5.8041635 75.006519
6.7277719 75.139683
7.7195434 75.1886
8.7794778 75.167805
9.9075753 75.088466
11.103836 74.95929
12.368259 74.787154
13.700845 74.577552
15.101595 74.334914
16.570507 74.06285
18.107582 73.764321
19.712821 73.441774
21.386222 73.097247
23.127786 72.732444
24.937514 72.348799
26.815404 71.947525
28.761457 71.52965
30.775673 71.096055
32.858053 70.647491
35.008595 70.184605
37.2273 69.707956
39.514168 69.21803
41.869199 68.715247
44.292394 68.199977
46.783751 67.672545
49.343271 67.133237
51.970954 66.58231
54.6668 66.019993
57.430809 65.446494
60.262981 64.862
63.163316 64.266687
66.131814 63.660717
69.168475 63.044242
72.273299 62.417408
75.446287 61.780355
78.687436 61.13322
81.996749 60.476139
85.374225 59.809244
88.819864 59.132672
92.333666 58.44656
95.915631 57.751048
99.565759 57.04628
103.28405 56.332405
107.0705 55.609578
110.92512 54.87796
114.8479 54.137719
118.83884 53.389032
122.89795 52.632083
127.02522 51.867067
131.22065 51.094186
135.48424 50.313653
139.816 49.525694
144.21592 48.730542
148.68401 47.928446
153.22025 47.119663
157.82466 46.304464
162.49724 45.483134
167.23797 44.655968
172.04687 43.823279
176.92393 42.985388
181.86916 42.142636
186.88254 41.295375
191.9641 40.443971
197.11381 39.588806
202.33169 38.730279
207.61772 37.868801
212.97193 37.0048
218.39429 36.138719
223.88482 35.271017
229.44351 34.402167
235.07037 33.532661
240.76539 32.663003
246.52857 31.793713
252.35991 30.925329
258.25942 30.058399
264.22708 29.19349
270.26292 28.331182
276.36691 27.472067
282.53907 26.616753
288.77939 25.765857
295.08788 24.920012
301.46452 24.079859
307.90933 23.246049
314.42231 22.419243
321.00344 21.600109
327.65274 20.789322
&
@target G1.S1
@type xy
1.0650467e-05 0.18441615
4.2601868e-05 0.18433224
0.018787423 0.14548992
0.071613737 0.091272435
0.15852154 0.056570531
0.27951085 0.036980218
0.43458164 0.025603323
0.62373393 0.018609808
0.84696771 0.014067247
1.104283 0.010973512
1.3956797 0.0087814063
1.721158 0.0071760338
2.0807178 0.0059673372
2.474359 0.0050357139
2.9020817 0.0043031144
3.363886 0.0037169731
3.8597717 0.003240899
4.3897389 0.0028490824
4.9537876 0.0025228238
5.5519178 0.0022483164
6.1841295 0.0020151921
6.8504227 0.0018155464
7.5507974 0.0016432694
8.2852536 0.0014935804
9.0537912 0.0013626956
9.8564104 0.0012475895
10.693111 0.00114582
11.563893 0.0010553989
12.468757 0.00097469402
13.407702 0.00090235602
14.380729 0.00083726135
15.387837 0.00077846859
16.429026 0.00072518418
17.504297 0.00067673547
18.61365 0.00063254931
19.757084 0.00059213494
20.9346 0.00055507022
22.146197 0.00052099045
23.391875 0.00048957926
24.671635 0.00046056118
25.985477 0.00043369546
27.3334 0.00040877097
28.715405 0.00038560198
30.131491 0.00036402457
31.581658 0.00034389366
33.065907 0.0003250805
34.584238 0.00030747051
36.13665 0.0002909615
37.723143 0.00027546208
39.343718 0.00026089035
40.998375 0.00024717279
42.687113 0.00023424319
44.409932 0.00022204189
46.166833 0.00021051499
47.957816 0.00019961371
49.78288 0.00018929385
51.642025 0.00017951528
53.535252 0.0001702415
55.46256 0.00016143929
57.42395 0.00015307834
59.419422 0.000145131
61.448975 0.00013757197
63.512609 0.00013037808
65.610325 0.00012352811
67.742122 0.00011700256
69.908001 0.00011078352
72.107962 0.00010485452
74.342004 9.9200354e-05
76.610127 9.3807021e-05
78.912332 8.8661569e-05
81.248618 8.3752019e-05
83.618986 7.9067268e-05
86.023435 7.4597014e-05
88.461966 7.0331677e-05
90.934578 6.6262336e-05
93.441272 6.2380665e-05
95.982048 5.8678881e-05
98.556904 5.5149692e-05
101.16584 5.1786247e-05
103.80886 4.8582099e-05
106.48596 4.5531162e-05
109.19715 4.2627678e-05
111.94241 3.9866182e-05
114.72176 3.7241474e-05
117.53518 3.4748591e-05
120.38269 3.2382783e-05
123.26428 3.0139489e-05
126.17995 2.8014318e-05
129.12971 2.6003029e-05
132.11354 2.4101517e-05
135.13146 2.2305794e-05
138.18346 2.061198e-05
141.26954 1.9016289e-05
144.3897 1.751502e-05
147.54394 1.6104546e-05
150.73226 1.478131e-05
153.95467 1.3541818e-05
157.21115 1.2382631e-05
160.50172 1.1300367e-05
163.82637 1.0291692e-05
&


==> plot1_enlo <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Tue Sep  7 11:14:13 2021"
@with string
@    string on
@    string loctype view
@    string 0.2047059, 0.250833333333
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.500000
@    string def "[unit 10\S-11\N MeV]"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.65, 17, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.244118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "i\Sth"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 3
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\SNLO\N\h{-1}\si\N   [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.2, 0.77
@    legend box color 1
@    legend box pattern 0
@    legend box linewidth 1.0
@    legend box linestyle 0
@    legend box fill color 0
@    legend box fill pattern 0
@    legend font 0
@    legend char size 1.750000
@    legend color 1
@    legend length 6
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 2.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  "c\snlo\N=-2"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 2
@    s1 line linewidth 4.0
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Cols 1:3"
@    s1 legend  "c\snlo\N=-4"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 0
@    s2 symbol size 1.000000
@    s2 symbol color 4
@    s2 symbol pattern 1
@    s2 symbol fill color 4
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 3
@    s2 line linewidth 2.5
@    s2 line color 4
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 4
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "Cols 1:3"
@    s2 legend  "c\snlo\N=-8"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 0
@    s3 symbol size 1.000000
@    s3 symbol color 3
@    s3 symbol pattern 1
@    s3 symbol fill color 3
@    s3 symbol fill pattern 0
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 5
@    s3 line linewidth 2.5
@    s3 line color 3
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 3
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "Cols 1:3"
@    s3 legend  "c\snlo\N=-15"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 0
@    s4 symbol size 1.000000
@    s4 symbol color 11
@    s4 symbol pattern 1
@    s4 symbol fill color 11
@    s4 symbol fill pattern 0
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 7
@    s4 line linewidth 2.0
@    s4 line color 11
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 11
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "Cols 1:3"
@    s4 legend  "c\snlo\N=-30"
@    s5 hidden false
@    s5 type xy
@    s5 symbol 1
@    s5 symbol size 0.500000
@    s5 symbol color 10
@    s5 symbol pattern 1
@    s5 symbol fill color 10
@    s5 symbol fill pattern 0
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 1
@    s5 line linestyle 2
@    s5 line linewidth 1.0
@    s5 line color 10
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 10
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "Cols 1:3"
@    s5 legend  "c\snlo\N=-60"
@    s6 hidden false
@    s6 type xy
@    s6 symbol 2
@    s6 symbol size 0.500000
@    s6 symbol color 13
@    s6 symbol pattern 1
@    s6 symbol fill color 13
@    s6 symbol fill pattern 0
@    s6 symbol linewidth 1.0
@    s6 symbol linestyle 1
@    s6 symbol char 65
@    s6 symbol char font 0
@    s6 symbol skip 0
@    s6 line type 1
@    s6 line linestyle 1
@    s6 line linewidth 1.0
@    s6 line color 13
@    s6 line pattern 1
@    s6 baseline type 0
@    s6 baseline off
@    s6 dropline off
@    s6 fill type 0
@    s6 fill rule 0
@    s6 fill color 1
@    s6 fill pattern 1
@    s6 avalue off
@    s6 avalue type 2
@    s6 avalue char size 1.000000
@    s6 avalue font 0
@    s6 avalue color 1
@    s6 avalue rot 0
@    s6 avalue format general
@    s6 avalue prec 3
@    s6 avalue prepend ""
@    s6 avalue append ""
@    s6 avalue offset 0.000000 , 0.000000
@    s6 errorbar on
@    s6 errorbar place both
@    s6 errorbar color 13
@    s6 errorbar pattern 1
@    s6 errorbar size 1.000000
@    s6 errorbar linewidth 1.0
@    s6 errorbar linestyle 1
@    s6 errorbar riser linewidth 1.0
@    s6 errorbar riser linestyle 1
@    s6 errorbar riser clip off
@    s6 errorbar riser clip length 0.100000
@    s6 comment "Cols 1:3"
@    s6 legend  "c\snlo\N=-120"
@target G0.S0
@type xy
1 -1.4396552e-06
2 -1.3866137e-05
3 -6.7134854e-05
4 -0.00025058733
5 -0.00085296148
6 -0.0028019842
7 -0.0074685469
8 -0.010480878
9 -0.0079712315
10 -0.0052908632
11 -0.0037973502
12 -0.0029738856
13 -0.0024812021
14 -0.0021623472
15 -0.0019424579
16 -0.001782968
17 -0.001662479
&
@target G0.S1
@type xy
1 -2.8793105e-06
2 -2.7732274e-05
3 -0.00013426971
4 -0.00050117466
5 -0.001705923
6 -0.0056039684
7 -0.014937094
8 -0.020961755
9 -0.015942463
10 -0.010581726
11 -0.0075947004
12 -0.0059477712
13 -0.0049624042
14 -0.0043246943
15 -0.0038849158
16 -0.003565936
17 -0.0033249581
&
@target G0.S2
@type xy
1 -5.758621e-06
2 -5.5464547e-05
3 -0.00026853942
4 -0.0010023493
5 -0.0034118459
6 -0.011207937
7 -0.029874188
8 -0.04192351
9 -0.031884926
10 -0.021163453
11 -0.015189401
12 -0.011895542
13 -0.0099248083
14 -0.0086493887
15 -0.0077698317
16 -0.0071318721
17 -0.0066499162
&
@target G0.S3
@type xy
1 -1.0797414e-05
2 -0.00010399603
3 -0.00050351141
4 -0.001879405
5 -0.0063972111
6 -0.021014881
7 -0.056014102
8 -0.078606582
9 -0.059784236
10 -0.039681474
11 -0.028480127
12 -0.022304142
13 -0.018609016
14 -0.016217604
15 -0.014568434
16 -0.01337226
17 -0.012468593
&
@target G0.S4
@type xy
1 -2.1594829e-05
2 -0.00020799205
3 -0.0010070228
4 -0.0037588099
5 -0.012794422
6 -0.042029763
7 -0.1120282
8 -0.15721316
9 -0.11956847
10 -0.079362947
11 -0.056960253
12 -0.044608284
13 -0.037218031
14 -0.032435208
15 -0.029136869
16 -0.02674452
17 -0.024937186
&
@target G0.S5
@type xy
1 -4.3189657e-05
2 -0.0004159841
3 -0.0020140456
4 -0.0075176199
5 -0.025588844
6 -0.084059526
7 -0.22405641
8 -0.31442633
9 -0.23913695
10 -0.15872589
11 -0.11392051
12 -0.089216568
13 -0.074436062
14 -0.064870415
15 -0.058273738
16 -0.05348904
17 -0.049874371
&
@target G0.S6
@type xy
1 -8.6379315e-05
2 -0.00083196821
3 -0.0040280913
4 -0.01503524
5 -0.051177689
6 -0.16811905
7 -0.44811282
8 -0.62885265
9 -0.47827389
10 -0.31745179
11 -0.22784101
12 -0.17843314
13 -0.14887212
14 -0.12974083
15 -0.11654748
16 -0.10697808
17 -0.099748743
18 -0.094100365
&


==> plot2_enlo <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Sep 13 10:44:09 2021"
@with string
@    string on
@    string loctype view
@    string 0.88, 0.8827451
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.250000
@    string def "All in unit: 10\S-11\N MeV\S-4"
@with string
@    string on
@    string loctype view
@    string 0.176470588235, 0.310049019608
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.250000
@    string def "c\slo\N=-250"
@with string
@    string on
@    string loctype view
@    string 0.831274509804, 0.312745098039
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.250000
@    string def "c\slo\N=-200"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.65, 17, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 0.605882, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "i\Sth"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\SNLO\N\h{-1}\si\N  [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.4, 0.58
@    legend box color 1
@    legend box pattern 0
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 0
@    legend font 0
@    legend char size 1.250000
@    legend color 1
@    legend length 3
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 2.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  "c\snlo\N=-2"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 2
@    s1 line linewidth 3.5
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Cols 1:3"
@    s1 legend  "c\snlo\N=-4"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 0
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 3
@    s2 line linewidth 2.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "Cols 1:3"
@    s2 legend  "c\snlo\N=-8"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 0
@    s3 symbol size 1.000000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 0
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 5
@    s3 line linewidth 2.0
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "Cols 1:3"
@    s3 legend  "c\snlo\N=-15"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 3
@    s4 symbol size 0.500000
@    s4 symbol color 11
@    s4 symbol pattern 1
@    s4 symbol fill color 11
@    s4 symbol fill pattern 0
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 7
@    s4 line linewidth 2.0
@    s4 line color 11
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 11
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "Cols 1:3"
@    s4 legend  "c\snlo\N=-30"
@    s5 hidden false
@    s5 type xy
@    s5 symbol 1
@    s5 symbol size 0.500000
@    s5 symbol color 10
@    s5 symbol pattern 1
@    s5 symbol fill color 10
@    s5 symbol fill pattern 0
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 1
@    s5 line linestyle 2
@    s5 line linewidth 1.0
@    s5 line color 10
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 10
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "Cols 1:3"
@    s5 legend  "c\snlo\N=-60"
@    s6 hidden false
@    s6 type xy
@    s6 symbol 2
@    s6 symbol size 0.500000
@    s6 symbol color 13
@    s6 symbol pattern 1
@    s6 symbol fill color 13
@    s6 symbol fill pattern 0
@    s6 symbol linewidth 1.0
@    s6 symbol linestyle 1
@    s6 symbol char 65
@    s6 symbol char font 0
@    s6 symbol skip 0
@    s6 line type 1
@    s6 line linestyle 1
@    s6 line linewidth 1.0
@    s6 line color 13
@    s6 line pattern 1
@    s6 baseline type 0
@    s6 baseline off
@    s6 dropline off
@    s6 fill type 0
@    s6 fill rule 0
@    s6 fill color 1
@    s6 fill pattern 1
@    s6 avalue off
@    s6 avalue type 2
@    s6 avalue char size 1.000000
@    s6 avalue font 0
@    s6 avalue color 1
@    s6 avalue rot 0
@    s6 avalue format general
@    s6 avalue prec 3
@    s6 avalue prepend ""
@    s6 avalue append ""
@    s6 avalue offset 0.000000 , 0.000000
@    s6 errorbar on
@    s6 errorbar place both
@    s6 errorbar color 13
@    s6 errorbar pattern 1
@    s6 errorbar size 1.000000
@    s6 errorbar linewidth 1.0
@    s6 errorbar linestyle 1
@    s6 errorbar riser linewidth 1.0
@    s6 errorbar riser linestyle 1
@    s6 errorbar riser clip off
@    s6 errorbar riser clip length 0.100000
@    s6 comment "Cols 1:3"
@    s6 legend  "c\snlo\N=-120"
@g1 on
@g1 hidden false
@g1 type XY
@g1 stacked false
@g1 bar hgap 0.000000
@g1 fixedpoint off
@g1 fixedpoint type 0
@g1 fixedpoint xy 0.000000, 0.000000
@g1 fixedpoint format general general
@g1 fixedpoint prec 6, 6
@with g1
@    world 11, -0.65, 21, 0
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.788235, 0.150000, 1.244118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "i\Sth"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\SNLO\N\h{-1}\si\N  [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 1.03, 0.51
@    legend box color 1
@    legend box pattern 0
@    legend box linewidth 1.0
@    legend box linestyle 0
@    legend box fill color 0
@    legend box fill pattern 0
@    legend font 0
@    legend char size 1.250000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 2.0
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  "c\snlo\N=-52"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 2
@    s1 line linewidth 4.0
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Cols 1:3"
@    s1 legend  "c\snlo\N=-54"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 0
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 3
@    s2 line linewidth 2.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "Cols 1:3"
@    s2 legend  "c\snlo\N=-58"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 0
@    s3 symbol size 1.000000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 0
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 5
@    s3 line linewidth 2.0
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "Cols 1:3"
@    s3 legend  "c\snlo\N=-65"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 3
@    s4 symbol size 0.500000
@    s4 symbol color 11
@    s4 symbol pattern 1
@    s4 symbol fill color 11
@    s4 symbol fill pattern 0
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 7
@    s4 line linewidth 2.0
@    s4 line color 11
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 11
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "Cols 1:3"
@    s4 legend  "c\snlo\N=-80"
@    s5 hidden false
@    s5 type xy
@    s5 symbol 1
@    s5 symbol size 0.500000
@    s5 symbol color 10
@    s5 symbol pattern 1
@    s5 symbol fill color 10
@    s5 symbol fill pattern 0
@    s5 symbol linewidth 1.0
@    s5 symbol linestyle 1
@    s5 symbol char 65
@    s5 symbol char font 0
@    s5 symbol skip 0
@    s5 line type 1
@    s5 line linestyle 2
@    s5 line linewidth 1.0
@    s5 line color 10
@    s5 line pattern 1
@    s5 baseline type 0
@    s5 baseline off
@    s5 dropline off
@    s5 fill type 0
@    s5 fill rule 0
@    s5 fill color 1
@    s5 fill pattern 1
@    s5 avalue off
@    s5 avalue type 2
@    s5 avalue char size 1.000000
@    s5 avalue font 0
@    s5 avalue color 1
@    s5 avalue rot 0
@    s5 avalue format general
@    s5 avalue prec 3
@    s5 avalue prepend ""
@    s5 avalue append ""
@    s5 avalue offset 0.000000 , 0.000000
@    s5 errorbar on
@    s5 errorbar place both
@    s5 errorbar color 10
@    s5 errorbar pattern 1
@    s5 errorbar size 1.000000
@    s5 errorbar linewidth 1.0
@    s5 errorbar linestyle 1
@    s5 errorbar riser linewidth 1.0
@    s5 errorbar riser linestyle 1
@    s5 errorbar riser clip off
@    s5 errorbar riser clip length 0.100000
@    s5 comment "Cols 1:3"
@    s5 legend  "c\snlo\N=-110"
@    s6 hidden false
@    s6 type xy
@    s6 symbol 2
@    s6 symbol size 0.500000
@    s6 symbol color 13
@    s6 symbol pattern 1
@    s6 symbol fill color 13
@    s6 symbol fill pattern 0
@    s6 symbol linewidth 1.0
@    s6 symbol linestyle 1
@    s6 symbol char 65
@    s6 symbol char font 0
@    s6 symbol skip 0
@    s6 line type 1
@    s6 line linestyle 1
@    s6 line linewidth 1.0
@    s6 line color 13
@    s6 line pattern 1
@    s6 baseline type 0
@    s6 baseline off
@    s6 dropline off
@    s6 fill type 0
@    s6 fill rule 0
@    s6 fill color 1
@    s6 fill pattern 1
@    s6 avalue off
@    s6 avalue type 2
@    s6 avalue char size 1.000000
@    s6 avalue font 0
@    s6 avalue color 1
@    s6 avalue rot 0
@    s6 avalue format general
@    s6 avalue prec 3
@    s6 avalue prepend ""
@    s6 avalue append ""
@    s6 avalue offset 0.000000 , 0.000000
@    s6 errorbar on
@    s6 errorbar place both
@    s6 errorbar color 13
@    s6 errorbar pattern 1
@    s6 errorbar size 1.000000
@    s6 errorbar linewidth 1.0
@    s6 errorbar linestyle 1
@    s6 errorbar riser linewidth 1.0
@    s6 errorbar riser linestyle 1
@    s6 errorbar riser clip off
@    s6 errorbar riser clip length 0.100000
@    s6 comment "Cols 1:3"
@    s6 legend  "c\snlo\N=-170"
@target G0.S0
@type xy
0 -1.4396552e-06
1 -1.3866137e-05
2 -6.7134854e-05
3 -0.00025058733
4 -0.00085296148
5 -0.0028019842
6 -0.0074685469
7 -0.010480878
8 -0.0079712315
9 -0.0052908632
10 -0.0037973502
11 -0.0029738856
12 -0.0024812021
13 -0.0021623472
14 -0.0019424579
15 -0.001782968
16 -0.001662479
&
@target G0.S1
@type xy
0 -2.8793105e-06
1 -2.7732274e-05
2 -0.00013426971
3 -0.00050117466
4 -0.001705923
5 -0.0056039684
6 -0.014937094
7 -0.020961755
8 -0.015942463
9 -0.010581726
10 -0.0075947004
11 -0.0059477712
12 -0.0049624042
13 -0.0043246943
14 -0.0038849158
15 -0.003565936
16 -0.0033249581
&
@target G0.S2
@type xy
0 -5.758621e-06
1 -5.5464547e-05
2 -0.00026853942
3 -0.0010023493
4 -0.0034118459
5 -0.011207937
6 -0.029874188
7 -0.04192351
8 -0.031884926
9 -0.021163453
10 -0.015189401
11 -0.011895542
12 -0.0099248083
13 -0.0086493887
14 -0.0077698317
15 -0.0071318721
16 -0.0066499162
&
@target G0.S3
@type xy
0 -1.0797414e-05
1 -0.00010399603
2 -0.00050351141
3 -0.001879405
4 -0.0063972111
5 -0.021014881
6 -0.056014102
7 -0.078606582
8 -0.059784236
9 -0.039681474
10 -0.028480127
11 -0.022304142
12 -0.018609016
13 -0.016217604
14 -0.014568434
15 -0.01337226
16 -0.012468593
&
@target G0.S4
@type xy
0 -2.1594829e-05
1 -0.00020799205
2 -0.0010070228
3 -0.0037588099
4 -0.012794422
5 -0.042029763
6 -0.1120282
7 -0.15721316
8 -0.11956847
9 -0.079362947
10 -0.056960253
11 -0.044608284
12 -0.037218031
13 -0.032435208
14 -0.029136869
15 -0.02674452
16 -0.024937186
&
@target G0.S5
@type xy
0 -4.3189657e-05
1 -0.0004159841
2 -0.0020140456
3 -0.0075176199
4 -0.025588844
5 -0.084059526
6 -0.22405641
7 -0.31442633
8 -0.23913695
9 -0.15872589
10 -0.11392051
11 -0.089216568
12 -0.074436062
13 -0.064870415
14 -0.058273738
15 -0.05348904
16 -0.049874371
&
@target G0.S6
@type xy
0 -8.6379315e-05
1 -0.00083196821
2 -0.0040280913
3 -0.01503524
4 -0.051177689
5 -0.16811905
6 -0.44811282
7 -0.62885265
8 -0.47827389
9 -0.31745179
10 -0.22784101
11 -0.17843314
12 -0.14887212
13 -0.12974083
14 -0.11654748
15 -0.10697808
16 -0.099748743
17 -0.094100365
&
@target G1.S0
@type xy
0 -3.3565677e-06
1 -2.9287762e-05
2 -0.00012073697
3 -0.00035462767
4 -0.000860675
5 -0.001853677
6 -0.0036866062
7 -0.0069319175
8 -0.01248569
9 -0.021631477
10 -0.035836094
11 -0.055800424
12 -0.079559217
13 -0.10140171
14 -0.11486096
15 -0.11781537
16 -0.11305258
17 -0.10466766
18 -0.095525048
19 -0.086999443
20 -0.079546678
21 -0.07319839
&
@target G1.S1
@type xy
0 -3.4856665e-06
1 -3.0414215e-05
2 -0.0001253807
3 -0.0003682672
4 -0.00089377789
5 -0.0019249722
6 -0.0038283988
7 -0.0071985297
8 -0.012965909
9 -0.022463457
10 -0.037214405
11 -0.057946594
12 -0.082619187
13 -0.10530177
14 -0.11927869
15 -0.12234673
16 -0.11740076
17 -0.10869334
18 -0.099199089
19 -0.090345575
20 -0.082606165
21 -0.076013713
&
@target G1.S2
@type xy
0 -3.743864e-06
1 -3.2667119e-05
2 -0.00013466816
3 -0.00039554625
4 -0.00095998366
5 -0.0020675628
6 -0.0041119839
7 -0.0077317542
8 -0.013926347
9 -0.024127417
10 -0.039971028
11 -0.062238935
12 -0.088739127
13 -0.1131019
14 -0.12811415
15 -0.13140946
16 -0.12609711
17 -0.1167447
18 -0.10654717
19 -0.09703784
20 -0.08872514
21 -0.081644358
&
@target G1.S3
@type xy
0 -4.1957097e-06
1 -3.6609703e-05
2 -0.00015092121
3 -0.00044328459
4 -0.0010758438
5 -0.0023170962
6 -0.0046082578
7 -0.0086648969
8 -0.015607113
9 -0.027039347
10 -0.044795117
11 -0.06975053
12 -0.099449022
13 -0.12675213
14 -0.1435762
15 -0.14726922
16 -0.14131573
17 -0.13083458
18 -0.11940631
19 -0.1087493
20 -0.099433347
21 -0.091497988
&
@target G1.S4
@type xy
0 -5.1639503e-06
1 -4.5058096e-05
2 -0.00018574919
3 -0.00054558103
4 -0.0013241154
5 -0.0028518107
6 -0.0056717019
7 -0.010664488
8 -0.019208754
9 -0.033279196
10 -0.055132452
11 -0.085846806
12 -0.1223988
13 -0.15600262
14 -0.17670917
15 -0.18125442
16 -0.17392705
17 -0.16102717
18 -0.14696161
19 -0.1338453
20 -0.1223795
21 -0.11261291
&
@target G1.S5
@type xy
0 -7.1004317e-06
1 -6.1954882e-05
2 -0.00025540513
3 -0.00075017392
4 -0.0018206587
5 -0.0039212397
6 -0.0077985901
7 -0.014663672
8 -0.026412037
9 -0.045758894
10 -0.075807121
11 -0.11803936
12 -0.16829834
13 -0.21450361
14 -0.24297511
15 -0.24922483
16 -0.23914969
17 -0.22141236
18 -0.20207222
19 -0.18403728
20 -0.16827182
21 -0.15484275
&
@target G1.S6
@type xy
0 -1.0973394e-05
1 -9.5748454e-05
2 -0.00039471702
3 -0.0011593597
4 -0.0028137452
5 -0.0060600977
6 -0.012052367
7 -0.022662038
8 -0.040818602
9 -0.070718291
10 -0.11715646
11 -0.18242446
12 -0.26009744
13 -0.33150557
14 -0.37550699
15 -0.38516565
16 -0.36959498
17 -0.34218274
18 -0.31229343
19 -0.28442126
20 -0.26005645
21 -0.23930243
&


==> plot_argand3p0 <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Nov  8 14:50:32 2021"
@with string
@    string on
@    string loctype view
@    string 0.457107843137, 0.753676470588
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.500000
@    string def "E\sR\N=0.53 MeV, \xG\0=0.23 MeV"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world -0.52, -0.02, 0.52, 1.02
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.194118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "Re[f]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.1
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Im[f]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.52, 0.6
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.500000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 2
@    s2 symbol pattern 1
@    s2 symbol fill color 2
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 0
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 2
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/mares/jerry/test_per/1"
@    s2 legend  "Resonance"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 1
@    s3 symbol size 0.500000
@    s3 symbol color 1
@    s3 symbol pattern 1
@    s3 symbol fill color 1
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 0
@    s3 line linestyle 0
@    s3 line linewidth 1.0
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 1
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "/home/mares/jerry/test_per/f_3p0_c1"
@    s3 legend  "f[E]"
@target G0.S2
@type xy
0 1
&
@target G0.S3
@type xy
2.8935221e-05 8.3724699e-10
0.00023295292 5.4267066e-08
0.00079462681 6.3143216e-07
0.0019121639 3.656384e-06
0.0038089355 1.45082e-05
0.0067453264 4.5501499e-05
0.011034154 0.00012176738
0.01706142 0.00029117682
0.025314927 0.00064125676
0.036424383 0.0013285006
0.051217979 0.0026301994
0.070801676 0.0050382614
0.096666247 0.0094333514
0.13081612 0.017416181
0.17586688 0.031949958
0.23488927 0.058607847
0.31022341 0.10787574
0.39889615 0.19853382
0.47939653 0.35794732
0.48997224 0.59963537
0.34940687 0.85765184
0.083684471 0.99294717
-0.16657079 0.97143841
-0.32831208 0.87710897
-0.41606145 0.77729564
-0.46050367 0.69477261
-0.48233697 0.63172337
-0.49275227 0.5848245
-0.49746421 0.5502927
-0.49937142 0.52506357
-0.49995288 0.50686409
-0.49996456 0.49404729
-0.49978737 0.48541972
-0.49960416 0.48010821
-0.49949192 0.47746514
-0.49947085 0.47700289
-0.499531 0.47834866
-0.49964693 0.48121307
-0.49978586 0.4853682
-0.49991223 0.49063192
-0.49999012 0.49685672
-0.49998462 0.50392146
&


==> plot_cro <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Tue Aug 31 17:20:44 2021"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, 0, 1, 2.4
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.244118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "E\scm\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\xs\0(\S3\NP\s0\N) [MeV\S-2\N]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.3
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.77, 0.92
@    legend box color 1
@    legend box pattern 0
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 0
@    legend font 0
@    legend char size 1.250000
@    legend color 1
@    legend length 7
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 2.5
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "Cols 1:3"
@    s0 legend  "c\snlo\N=-2*10\S-11\N MeV\S-4"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 2
@    s1 symbol pattern 1
@    s1 symbol fill color 2
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 3
@    s1 line linewidth 2.5
@    s1 line color 2
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 2
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Cols 1:3"
@    s1 legend  "c\snlo\N=-4*10\S-11\N MeV\S-4"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 0
@    s2 symbol size 1.000000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 5
@    s2 line linewidth 2.5
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "Cols 1:3"
@    s2 legend  "c\snlo\N=-8*10\S-11\N MeV\S-4"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 0
@    s3 symbol size 1.000000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 0
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 7
@    s3 line linewidth 2.5
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "Cols 1:3"
@    s3 legend  "c\snlo\N=-15*10\S-11\N MeV\S-4"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 0
@    s4 symbol size 1.000000
@    s4 symbol color 8
@    s4 symbol pattern 1
@    s4 symbol fill color 8
@    s4 symbol fill pattern 0
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 2
@    s4 line linewidth 3.5
@    s4 line color 8
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 8
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "Cols 1:3"
@    s4 legend  "c\snlo\N=-30*10\S-11\N MeV\S-4"
@target G0.S0
@type xy
4.2601867e-05 6.0685475e-11
0.00017040747 9.7150147e-10
0.0003834168 4.9227356e-09
0.00068162986 1.557826e-08
0.0010650467 3.8095725e-08
0.0015336672 7.9155046e-08
0.0020874915 1.4699539e-07
0.0027265195 2.5146093e-07
0.0034507512 4.0405578e-07
0.0042601867 6.1800841e-07
0.0051548258 9.0834615e-07
0.0061346688 1.2919803e-06
0.0071997154 1.7878025e-06
0.0083499658 2.4167933e-06
0.00958542 3.2021431e-06
0.010906078 4.169388e-06
0.012311939 5.3465593e-06
0.013803005 6.7643503e-06
0.015379274 8.4563003e-06
0.017040747 1.0458997e-05
0.018787423 1.2812302e-05
0.020619303 1.5559596e-05
0.022536387 1.8748051e-05
0.024538675 2.2428929e-05
0.026626167 2.6657914e-05
0.028798862 3.1495469e-05
0.031056761 3.700724e-05
0.033399863 4.3264494e-05
0.03582817 5.0344598e-05
0.03834168 5.8331561e-05
0.040940394 6.7316612e-05
0.043624311 7.7398855e-05
0.046393433 8.8685982e-05
0.049247758 0.00010129506
0.052187286 0.00011535342
0.055212019 0.0001309996
0.058321955 0.00014838444
0.061517095 0.00016767223
0.064797439 0.0001890421
0.068162986 0.00021268939
0.071613738 0.00023882735
0.075149693 0.0002676889
0.078770851 0.00029952868
0.082477214 0.00033462526
0.08626878 0.00037328368
0.09014555 0.00041583821
0.094107523 0.00046265553
0.0981547 0.00051413821
0.10228708 0.00057072865
0.10650467 0.00063291349
0.11080745 0.00070122857
0.11519545 0.00077626455
0.11966864 0.00085867312
0.12422704 0.00094917419
0.12887065 0.0010485638
0.13359945 0.0011577233
0.13841346 0.0012776293
0.14331268 0.0014093658
0.1482971 0.0015541366
0.15336672 0.001713281
0.15852155 0.00188829
0.16376157 0.0020808262
0.16908681 0.0022927453
0.17449725 0.002526121
0.17999289 0.0027832739
0.18557373 0.0030668029
0.19123978 0.0033796229
0.19699103 0.003725006
0.20282749 0.0041066292
0.20874915 0.0045286285
0.21475601 0.0049956601
0.22084808 0.0055129692
0.22702535 0.0060864679
0.23328782 0.0067228225
0.2396355 0.0074295498
0.24606838 0.0082151246
0.25258647 0.0090890952
0.25918976 0.010062208
0.26587825 0.011146538
0.27265195 0.012355618
0.27951085 0.013704567
0.28645495 0.015210192
0.29348426 0.016891068
0.30059877 0.01876755
0.30779849 0.020861696
0.3150834 0.023197061
0.32245353 0.025798277
0.32990885 0.028690371
0.33744938 0.031897695
0.34507512 0.035442366
0.35278606 0.039342087
0.3605822 0.043607227
0.36846354 0.048237084
0.37643009 0.053215338
0.38448185 0.058504866
0.3926188 0.064042365
0.40084096 0.069733536
0.40914833 0.075450008
0.41754089 0.081029486
0.42601867 0.086280693
0.43458164 0.090994299
0.44322982 0.094960008
0.4519632 0.097988358
0.46078179 0.09993394
0.46968558 0.10071537
0.47867457 0.10032729
0.48774877 0.098841033
0.49690817 0.096393778
0.50615278 0.093168624
0.51548258 0.089370544
0.5248976 0.085203319
0.53439781 0.080851396
0.54398323 0.076468596
0.55365386 0.072173555
0.56340968 0.068050493
0.57325072 0.064153387
0.58317695 0.060511744
0.59318839 0.057136628
0.60328503 0.054026113
0.61346688 0.051169771
0.62373393 0.048552128
0.63408618 0.046155156
0.64452364 0.043959988
0.6550463 0.041948023
0.66565416 0.040101592
0.67634723 0.038404316
0.6871255 0.036841258
0.69798898 0.035398948
0.70893766 0.034065328
0.71997154 0.032829655
0.73109063 0.031682387
0.74229492 0.030615053
0.75358442 0.029620144
0.76495911 0.028690992
0.77641902 0.027821676
0.78796412 0.027006926
0.79959443 0.026242044
0.81130995 0.025522835
0.82311066 0.024845544
0.83499658 0.0242068
0.84696771 0.023603576
0.85902404 0.023033141
0.87116557 0.02249303
0.8833923 0.021981012
0.89570424 0.021495064
0.90810139 0.021033345
0.92058373 0.02059418
0.93315128 0.020176042
0.94580404 0.019777531
0.958542 0.019397369
0.97136516 0.01903438
0.98427352 0.018687486
0.99726709 0.018355694
1.0103459 0.018038087
1.0235098 0.01773382
1.036759 0.017442111
1.0500934 0.017162237
1.063513 0.016893526
1.0770178 0.016635355
1.0906078 0.016387147
1.104283 0.01614836
1.1180434 0.015918495
1.131889 0.015697083
1.1458198 0.015483686
1.1598358 0.015277896
1.173937 0.015079331
1.1881235 0.014887632
1.2023951 0.014702465
1.2167519 0.014523515
1.2311939 0.014350485
1.2457212 0.014183098
1.2603336 0.014021093
1.2750313 0.013864223
1.2898141 0.013712256
1.3046822 0.013564974
1.3196354 0.013422169
1.3346739 0.013283649
1.3497975 0.013149227
1.3650064 0.01301873
1.3803005 0.012891993
1.3956797 0.012768859
1.4111442 0.012649182
1.4266939 0.012532819
1.4423288 0.012419639
1.4580489 0.012309515
1.4738542 0.012202327
1.4897447 0.01209796
1.5057204 0.011996306
1.5217813 0.011897262
1.5379274 0.011800729
1.5541587 0.011706614
1.5704752 0.011614827
1.5868769 0.011525283
1.6033638 0.011437901
1.619936 0.011352603
1.6365933 0.011269316
1.6533358 0.011187967
1.6701636 0.011108491
1.6870765 0.011030822
1.7040747 0.010954897
1.721158 0.010880659
1.7383266 0.010808049
1.7555803 0.010737015
1.7729193 0.010667502
1.7903434 0.010599463
1.8078528 0.010532848
1.8254474 0.010467612
1.8431272 0.01040371
1.8608921 0.010341101
1.8787423 0.010279743
1.8966777 0.010219597
1.9146983 0.010160626
1.9328041 0.010102794
1.9509951 0.010046065
1.9692713 0.0099904067
1.9876327 0.0099357862
2.0060793 0.0098821726
2.0246111 0.0098295361
2.0432281 0.0097778477
2.0619303 0.0097270798
2.0807178 0.0096772055
2.0995904 0.009628199
2.1185482 0.0095800354
2.1375913 0.0095326906
2.1567195 0.0094861414
2.1759329 0.0094403654
2.1952316 0.0093953409
2.2146154 0.0093510469
2.2340845 0.0093074634
2.2536387 0.0092645707
2.2732782 0.0092223499
2.2930029 0.0091807827
2.3128127 0.0091398514
2.3327078 0.009099539
2.3526881 0.0090598288
2.3727536 0.0090207049
2.3929042 0.0089821516
2.4131401 0.0089441539
2.4334612 0.0089066973
2.4538675 0.0088697676
2.474359 0.0088333512
2.4949357 0.0087974346
2.5155976 0.0087620051
2.5363447 0.0087270502
2.557177 0.0086925577
2.5780946 0.0086585159
2.5990973 0.0086249134
2.6201852 0.0085917391
2.6413583 0.0085589821
2.6626167 0.0085266322
2.6839602 0.008494679
2.7053889 0.0084631129
2.7269029 0.008431924
2.748502 0.0084011032
2.7701864 0.0083706414
2.7919559 0.0083405298
2.8138107 0.0083107598
2.8357506 0.008281323
2.8577758 0.0082522114
2.8798862 0.0082234171
2.9020817 0.0081949323
2.9243625 0.0081667497
2.9467285 0.0081388619
2.9691797 0.0081112619
2.9917161 0.0080839427
3.0143377 0.0080568977
3.0370445 0.0080301202
3.0598365 0.0080036039
3.0827137 0.0079773426
3.1056761 0.0079513302
3.1287237 0.0079255609
3.1518565 0.0079000287
3.1750745 0.0078747282
3.1983777 0.0078496539
3.2217662 0.0078248003
3.2452398 0.0078001623
3.2687986 0.0077757348
3.2924427 0.0077515128
3.3161719 0.0077274916
3.3399863 0.0077036662
3.363886 0.0076800322
3.3878708 0.0076565851
3.4119409 0.0076333203
3.4360961 0.0076102337
3.4603366 0.007587321
3.4846623 0.0075645781
3.5090731 0.007542001
3.5335692 0.0075195858
3.5581505 0.0074973286
3.582817 0.0074752258
3.6075687 0.0074532736
3.6324055 0.0074314686
3.6573276 0.0074098071
3.6823349 0.0073882858
3.7074274 0.0073669013
3.7326051 0.0073456504
3.757868 0.0073245298
3.7832162 0.0073035365
3.8086495 0.0072826673
3.834168 0.0072619193
3.8597717 0.0072412896
3.8854606 0.0072207753
3.9112348 0.0072003735
3.9370941 0.0071800816
3.9630386 0.0071598968
3.9890684 0.0071398166
4.0151833 0.0071198382
4.0413835 0.0070999593
4.0676688 0.0070801774
4.0940394 0.0070604899
4.1204951 0.0070408947
4.1470361 0.0070213892
4.1736623 0.0070019714
4.2003736 0.0069826388
4.2271702 0.0069633895
4.254052 0.0069442211
4.281019 0.0069251317
4.3080711 0.0069061192
4.3352085 0.0068871816
4.3624311 0.0068683168
4.3897389 0.006849523
4.4171319 0.0068307984
4.4446101 0.0068121409
4.4721735 0.0067935489
4.4998221 0.0067750205
4.527556 0.006756554
4.555375 0.0067381476
4.5832792 0.0067197998
4.6112686 0.0067015089
4.6393433 0.0066832731
4.6675031 0.0066650911
4.6957481 0.0066469612
4.7240784 0.0066288819
4.7524938 0.0066108517
4.7809945 0.0065928691
4.8095803 0.0065749328
4.8382514 0.0065570413
4.8670076 0.0065391932
4.8958491 0.0065213873
4.9247758 0.0065036221
4.9537876 0.0064858964
4.9828847 0.0064682089
5.012067 0.0064505583
5.0413345 0.0064329435
5.0706872 0.0064153633
5.1001251 0.0063978163
5.1296481 0.0063803017
5.1592564 0.006362818
5.1889499 0.0063453644
5.2187286 0.0063279396
5.2485926 0.0063105427
5.2785417 0.0062931725
5.308576 0.0062758281
5.3386955 0.0062585085
5.3689002 0.0062412126
5.3991902 0.0062239396
5.4295653 0.0062066883
5.4600256 0.0061894581
5.4905712 0.0061722478
5.5212019 0.0061550567
5.5519178 0.0061378839
5.582719 0.0061207285
5.6136053 0.0061035896
5.6445769 0.0060864666
5.6756337 0.0060693585
5.7067756 0.0060522645
5.7380028 0.006035184
5.7693152 0.0060181161
5.8007127 0.0060010602
5.8321955 0.0059840154
5.8637635 0.0059669811
5.8954167 0.0059499566
5.9271551 0.0059329413
5.9589787 0.0059159344
5.9908875 0.0058989353
6.0228815 0.0058819433
6.0549607 0.005864958
6.0871251 0.0058479786
6.1193747 0.0058310045
6.1517095 0.0058140352
6.1841295 0.0057970702
6.2166348 0.0057801088
6.2492252 0.0057631505
6.2819008 0.0057461949
6.3146617 0.0057292413
6.3475077 0.0057122893
6.3804389 0.0056953384
6.4134554 0.0056783881
6.446557 0.0056614379
6.4797439 0.0056444875
6.513016 0.0056275363
6.5463732 0.005610584
6.5798157 0.00559363
6.6133433 0.0055766741
6.6469562 0.0055597157
6.6806543 0.0055427546
6.7144376 0.0055257903
6.7483061 0.0055088225
6.7822597 0.0054918508
6.8162986 0.005474875
&
@target G0.S1
@type xy
4.2601867e-05 7.204732e-11
0.00017040747 1.1534345e-09
0.0003834168 5.8449842e-09
0.00068162986 1.8498397e-08
0.0010650467 4.5241891e-08
0.0015336672 9.4016372e-08
0.0020874915 1.7462244e-07
0.0027265195 2.9877862e-07
0.0034507512 4.801912e-07
0.0042601867 7.3463639e-07
0.0051548258 1.0800553e-06
0.0061346688 1.5366629e-06
0.0071997154 2.1270707e-06
0.0083499658 2.8764267e-06
0.00958542 3.8125699e-06
0.010906078 4.9662053e-06
0.012311939 6.3710964e-06
0.013803005 8.0642806e-06
0.015379274 1.0086307e-05
0.017040747 1.24815e-05
0.018787423 1.5298249e-05
0.020619303 1.8589332e-05
0.022536387 2.241227e-05
0.024538675 2.6829717e-05
0.026626167 3.1909894e-05
0.028798862 3.7727065e-05
0.031056761 4.4362067e-05
0.033399863 5.1902886e-05
0.03582817 6.0445305e-05
0.03834168 7.0093611e-05
0.040940394 8.0961385e-05
0.043624311 9.3172364e-05
0.046393433 0.00010686141
0.049247758 0.00012217559
0.052187286 0.00013927532
0.055212019 0.00015833572
0.058321955 0.00017954808
0.061517095 0.00020312145
0.064797439 0.00022928448
0.068162986 0.00025828741
0.071613738 0.00029040436
0.075149693 0.00032593582
0.078770851 0.00036521148
0.082477214 0.00040859337
0.08626878 0.00045647938
0.09014555 0.00050930726
0.094107523 0.00056755903
0.0981547 0.00063176602
0.10228708 0.00070251452
0.10650467 0.0007804521
0.11080745 0.00086629484
0.11519545 0.00096083544
0.11966864 0.0010649524
0.12422704 0.0011796204
0.12887065 0.0013059223
0.13359945 0.0014450623
0.13841346 0.0015983815
0.14331268 0.001767375
0.1482971 0.0019537122
0.15336672 0.0021592588
0.15852155 0.0023861032
0.16376157 0.0026365859
0.16908681 0.0029133332
0.17449725 0.0032192963
0.17999289 0.0035577952
0.18557373 0.0039325701
0.19123978 0.0043478393
0.19699103 0.0048083665
0.20282749 0.0053195366
0.20874915 0.0058874441
0.21475601 0.0065189922
0.22084808 0.0072220074
0.22702535 0.0080053682
0.23328782 0.0088791517
0.2396355 0.0098547976
0.24606838 0.010945291
0.25258647 0.012165365
0.25918976 0.013531717
0.26587825 0.015063246
0.27265195 0.016781286
0.27951085 0.018709849
0.28645495 0.020875832
0.29348426 0.023309182
0.30059877 0.026042974
0.30779849 0.029113329
0.3150834 0.032559119
0.32245353 0.036421322
0.32990885 0.0407419
0.33744938 0.045562011
0.34507512 0.050919342
0.35278606 0.056844313
0.3605822 0.063354923
0.36846354 0.070450058
0.37643009 0.078101265
0.38448185 0.086243265
0.3926188 0.094763994
0.40084096 0.10349561
0.40914833 0.11220865
0.41754089 0.12061224
0.42601867 0.12836342
0.43458164 0.13508793
0.44322982 0.14041293
0.4519632 0.14400887
0.46078179 0.14563398
0.46968558 0.14517214
0.47867457 0.14265467
0.48774877 0.13825943
0.49690817 0.13228668
0.50615278 0.12511741
0.51548258 0.11716395
0.5248976 0.10882366
0.53439781 0.10044369
0.54398323 0.092300418
0.55365386 0.084593154
0.56340968 0.077448657
0.57325072 0.070932312
0.58317695 0.065062015
0.59318839 0.059821936
0.60328503 0.055174496
0.61346688 0.051069864
0.62373393 0.04745293
0.63408618 0.044268069
0.64452364 0.041462148
0.6550463 0.038986219
0.66565416 0.03679631
0.67634723 0.034853613
0.6871255 0.033124314
0.69798898 0.031579214
0.70893766 0.030193253
0.71997154 0.028945016
0.73109063 0.027816244
0.74229492 0.026791391
0.75358442 0.025857218
0.76495911 0.025002446
0.77641902 0.024217451
0.78796412 0.023494003
0.79959443 0.022825053
0.81130995 0.022204542
0.82311066 0.021627249
0.83499658 0.021088661
0.84696771 0.020584864
0.85902404 0.02011245
0.87116557 0.019668444
0.8833923 0.019250238
0.89570424 0.01885554
0.90810139 0.018482325
0.92058373 0.018128801
0.93315128 0.017793375
0.94580404 0.017474629
0.958542 0.017171292
0.97136516 0.016882225
0.98427352 0.016606404
0.99726709 0.016342902
1.0103459 0.016090882
1.0235098 0.015849585
1.036759 0.015618318
1.0500934 0.015396451
1.063513 0.015183406
1.0770178 0.014978654
1.0906078 0.014781711
1.104283 0.014592127
1.1180434 0.014409491
1.131889 0.014233422
1.1458198 0.014063565
1.1598358 0.013899594
1.173937 0.013741205
1.1881235 0.013588113
1.2023951 0.013440056
1.2167519 0.013296786
1.2311939 0.013158074
1.2457212 0.013023703
1.2603336 0.012893473
1.2750313 0.012767192
1.2898141 0.012644683
1.3046822 0.012525779
1.3196354 0.012410322
1.3346739 0.012298163
1.3497975 0.012189162
1.3650064 0.012083187
1.3803005 0.011980112
1.3956797 0.011879819
1.4111442 0.011782196
1.4266939 0.011687137
1.4423288 0.01159454
1.4580489 0.011504311
1.4738542 0.011416358
1.4897447 0.011330595
1.5057204 0.011246941
1.5217813 0.011165316
1.5379274 0.011085646
1.5541587 0.011007861
1.5704752 0.010931892
1.5868769 0.010857676
1.6033638 0.01078515
1.619936 0.010714256
1.6365933 0.010644938
1.6533358 0.010577141
1.6701636 0.010510815
1.6870765 0.010445909
1.7040747 0.010382378
1.721158 0.010320174
1.7383266 0.010259256
1.7555803 0.010199582
1.7729193 0.010141112
1.7903434 0.010083807
1.8078528 0.010027631
1.8254474 0.0099725484
1.8431272 0.0099185254
1.8608921 0.0098655295
1.8787423 0.0098135291
1.8966777 0.0097624941
1.9146983 0.0097123955
1.9328041 0.0096632054
1.9509951 0.0096148966
1.9692713 0.0095674434
1.9876327 0.0095208207
2.0060793 0.0094750044
2.0246111 0.0094299711
2.0432281 0.0093856985
2.0619303 0.0093421649
2.0807178 0.0092993494
2.0995904 0.0092572318
2.1185482 0.0092157925
2.1375913 0.0091750128
2.1567195 0.0091348744
2.1759329 0.0090953597
2.1952316 0.0090564517
2.2146154 0.0090181339
2.2340845 0.0089803903
2.2536387 0.0089432055
2.2732782 0.0089065647
2.2930029 0.0088704532
2.3128127 0.0088348571
2.3327078 0.0087997629
2.3526881 0.0087651573
2.3727536 0.0087310277
2.3929042 0.0086973616
2.4131401 0.008664147
2.4334612 0.0086313724
2.4538675 0.0085990265
2.474359 0.0085670983
2.4949357 0.0085355771
2.5155976 0.0085044527
2.5363447 0.008473715
2.557177 0.0084433543
2.5780946 0.0084133612
2.5990973 0.0083837264
2.6201852 0.008354441
2.6413583 0.0083254964
2.6626167 0.0082968841
2.6839602 0.008268596
2.7053889 0.0082406239
2.7269029 0.0082129602
2.748502 0.0081855974
2.7701864 0.0081585279
2.7919559 0.0081317448
2.8138107 0.008105241
2.8357506 0.0080790098
2.8577758 0.0080530445
2.8798862 0.0080273387
2.9020817 0.0080018862
2.9243625 0.0079766808
2.9467285 0.0079517166
2.9691797 0.0079269877
2.9917161 0.0079024886
3.0143377 0.0078782138
3.0370445 0.0078541577
3.0598365 0.0078303153
3.0827137 0.0078066813
3.1056761 0.0077832508
3.1287237 0.007760019
3.1518565 0.007736981
3.1750745 0.0077141323
3.1983777 0.0076914683
3.2217662 0.0076689845
3.2452398 0.0076466768
3.2687986 0.0076245408
3.2924427 0.0076025724
3.3161719 0.0075807677
3.3399863 0.0075591227
3.363886 0.0075376335
3.3878708 0.0075162965
3.4119409 0.0074951079
3.4360961 0.0074740642
3.4603366 0.0074531619
3.4846623 0.0074323975
3.5090731 0.0074117677
3.5335692 0.0073912693
3.5581505 0.007370899
3.582817 0.0073506536
3.6075687 0.0073305303
3.6324055 0.0073105258
3.6573276 0.0072906374
3.6823349 0.0072708622
3.7074274 0.0072511972
3.7326051 0.0072316399
3.757868 0.0072121875
3.7832162 0.0071928374
3.8086495 0.0071735869
3.834168 0.0071544337
3.8597717 0.0071353751
3.8854606 0.0071164089
3.9112348 0.0070975326
3.9370941 0.0070787439
3.9630386 0.0070600405
3.9890684 0.0070414202
4.0151833 0.0070228809
4.0413835 0.0070044204
4.0676688 0.0069860366
4.0940394 0.0069677274
4.1204951 0.006949491
4.1470361 0.0069313251
4.1736623 0.0069132281
4.2003736 0.0068951979
4.2271702 0.0068772327
4.254052 0.0068593308
4.281019 0.0068414902
4.3080711 0.0068237093
4.3352085 0.0068059864
4.3624311 0.0067883198
4.3897389 0.0067707079
4.4171319 0.0067531489
4.4446101 0.0067356414
4.4721735 0.0067181839
4.4998221 0.0067007747
4.527556 0.0066834124
4.555375 0.0066660955
4.5832792 0.0066488226
4.6112686 0.0066315924
4.6393433 0.0066144033
4.6675031 0.0065972542
4.6957481 0.0065801436
4.7240784 0.0065630702
4.7524938 0.0065460328
4.7809945 0.0065290301
4.8095803 0.0065120609
4.8382514 0.006495124
4.8670076 0.0064782182
4.8958491 0.0064613424
4.9247758 0.0064444954
4.9537876 0.0064276761
4.9828847 0.0064108834
5.012067 0.0063941163
5.0413345 0.0063773737
5.0706872 0.0063606546
5.1001251 0.0063439579
5.1296481 0.0063272827
5.1592564 0.006310628
5.1889499 0.0062939929
5.2187286 0.0062773764
5.2485926 0.0062607776
5.2785417 0.0062441956
5.308576 0.0062276296
5.3386955 0.0062110786
5.3689002 0.0061945419
5.3991902 0.0061780185
5.4295653 0.0061615078
5.4600256 0.0061450088
5.4905712 0.0061285209
5.5212019 0.0061120432
5.5519178 0.0060955751
5.582719 0.0060791157
5.6136053 0.0060626644
5.6445769 0.0060462205
5.6756337 0.0060297832
5.7067756 0.006013352
5.7380028 0.005996926
5.7693152 0.0059805048
5.8007127 0.0059640877
5.8321955 0.005947674
5.8637635 0.0059312631
5.8954167 0.0059148545
5.9271551 0.0058984476
5.9589787 0.0058820418
5.9908875 0.0058656366
6.0228815 0.0058492314
6.0549607 0.0058328256
6.0871251 0.0058164189
6.1193747 0.0058000107
6.1517095 0.0057836004
6.1841295 0.0057671877
6.2166348 0.0057507719
6.2492252 0.0057343528
6.2819008 0.0057179298
6.3146617 0.0057015025
6.3475077 0.0056850705
6.3804389 0.0056686334
6.4134554 0.0056521908
6.446557 0.0056357422
6.4797439 0.0056192873
6.513016 0.0056028258
6.5463732 0.0055863572
6.5798157 0.0055698813
6.6133433 0.0055533976
6.6469562 0.0055369059
6.6806543 0.0055204058
6.7144376 0.0055038971
6.7483061 0.0054873794
6.7822597 0.0054708524
6.8162986 0.0054543159
&
@target G0.S2
@type xy
4.2601867e-05 9.7694076e-11
0.00017040747 1.5641169e-09
0.0003834168 7.9268878e-09
0.00068162986 2.5090764e-08
0.0010650467 6.1375955e-08
0.0015336672 1.2757223e-07
0.0020874915 2.3700926e-07
0.0027265195 4.0564387e-07
0.0034507512 6.5216485e-07
0.0042601867 9.9811638e-07
0.0051548258 1.468041e-06
0.0061346688 2.0896436e-06
0.0071997154 2.8939778e-06
0.0083499658 3.915656e-06
0.00958542 5.1930862e-06
0.010906078 6.7687361e-06
0.012311939 8.6894287e-06
0.013803005 1.1006671e-05
0.015379274 1.3777018e-05
0.017040747 1.706248e-05
0.018787423 2.0930971e-05
0.020619303 2.5456808e-05
0.022536387 3.0721262e-05
0.024538675 3.681317e-05
0.026626167 4.3829611e-05
0.028798862 5.1876659e-05
0.031056761 6.1070213e-05
0.033399863 7.1536921e-05
0.03582817 8.3415199e-05
0.03834168 9.6856373e-05
0.040940394 0.00011202594
0.043624311 0.00012910495
0.046393433 0.00014829161
0.049247758 0.00016980297
0.052187286 0.0001938769
0.055212019 0.00022077424
0.058321955 0.00025078118
0.061517095 0.00028421201
0.064797439 0.00032141209
0.068162986 0.00036276127
0.071613738 0.00040867765
0.075149693 0.00045962186
0.078770851 0.00051610183
0.082477214 0.0005786782
0.08626878 0.00064797035
0.09014555 0.00072466331
0.094107523 0.00080951546
0.0981547 0.00090336732
0.10228708 0.0010071514
0.10650467 0.0011219036
0.11080745 0.0012487759
0.11519545 0.0013890508
0.11966864 0.0015441581
0.12422704 0.0017156937
0.12887065 0.0019054411
0.13359945 0.0021153962
0.13841346 0.0023477955
0.14331268 0.0026051484
0.1482971 0.0028902746
0.15336672 0.0032063467
0.15852155 0.0035569396
0.16376157 0.003946087
0.16908681 0.0043783467
0.17449725 0.0048588767
0.17999289 0.0053935215
0.18557373 0.0059889138
0.19123978 0.0066525906
0.19699103 0.0073931283
0.20282749 0.0082202985
0.20874915 0.0091452484
0.21475601 0.010180709
0.22084808 0.011341235
0.22702535 0.012643481
0.23328782 0.014106517
0.2396355 0.01575219
0.24606838 0.017605533
0.25258647 0.019695226
0.25918976 0.022054102
0.26587825 0.024719715
0.27265195 0.02773493
0.27951085 0.031148547
0.28645495 0.03501591
0.29348426 0.039399456
0.30059877 0.044369128
0.30779849 0.050002533
0.3150834 0.056384685
0.32245353 0.063607086
0.32990885 0.07176585
0.33744938 0.080958439
0.34507512 0.091278512
0.35278606 0.10280828
0.3605822 0.11560774
0.36846354 0.12970028
0.37643009 0.14505435
0.38448185 0.16156165
0.3926188 0.17901316
0.40084096 0.19707613
0.40914833 0.21527661
0.41754089 0.23299442
0.42601867 0.24947793
0.43458164 0.26388532
0.44322982 0.27535484
0.4519632 0.28309939
0.46078179 0.2865119
0.46968558 0.2852603
0.47867457 0.27934871
0.48774877 0.26912743
0.49690817 0.25524709
0.50615278 0.2385675
0.51548258 0.22004347
0.5248976 0.20061313
0.53439781 0.18110913
0.54398323 0.16220366
0.55365386 0.14438744
0.56340968 0.12797627
0.57325072 0.11313505
0.58317695 0.099909979
0.59318839 0.088261642
0.60328503 0.078094537
0.61346688 0.069280957
0.62373393 0.061678847
0.63408618 0.055144221
0.64452364 0.049539128
0.6550463 0.044736267
0.66565416 0.040621222
0.67634723 0.037093091
0.6871255 0.034064131
0.69798898 0.031458828
0.70893766 0.029212683
0.71997154 0.027270912
0.73109063 0.025587165
0.74229492 0.024122332
0.75358442 0.022843465
0.76495911 0.021722832
0.77641902 0.020737094
0.78796412 0.019866604
0.79959443 0.019094809
0.81130995 0.018407749
0.82311066 0.017793631
0.83499658 0.017242481
0.84696771 0.016745843
0.85902404 0.016296537
0.87116557 0.015888454
0.8833923 0.015516382
0.89570424 0.015175866
0.90810139 0.01486309
0.92058373 0.014574775
0.93315128 0.014308097
0.94580404 0.014060621
0.958542 0.013830238
0.97136516 0.013615118
0.98427352 0.013413671
0.99726709 0.013224508
1.0103459 0.013046417
1.0235098 0.012878335
1.036759 0.012719328
1.0500934 0.012568571
1.063513 0.012425339
1.0770178 0.012288987
1.0906078 0.012158944
1.104283 0.012034701
1.1180434 0.011915803
1.131889 0.011801846
1.1458198 0.011692463
1.1598358 0.011587329
1.173937 0.011486148
1.1881235 0.011388653
1.2023951 0.011294603
1.2167519 0.011203779
1.2311939 0.011115982
1.2457212 0.011031029
1.2603336 0.010948756
1.2750313 0.010869009
1.2898141 0.01079165
1.3046822 0.010716549
1.3196354 0.010643589
1.3346739 0.01057266
1.3497975 0.010503662
1.3650064 0.0104365
1.3803005 0.010371087
1.3956797 0.010307343
1.4111442 0.010245192
1.4266939 0.010184563
1.4423288 0.010125391
1.4580489 0.010067614
1.4738542 0.010011173
1.4897447 0.0099560155
1.5057204 0.009902089
1.5217813 0.0098493456
1.5379274 0.0097977397
1.5541587 0.0097472284
1.5704752 0.009697771
1.5868769 0.0096493289
1.6033638 0.0096018657
1.619936 0.0095553466
1.6365933 0.0095097388
1.6533358 0.0094650109
1.6701636 0.0094211331
1.6870765 0.009378077
1.7040747 0.0093358154
1.721158 0.0092943224
1.7383266 0.0092535734
1.7555803 0.0092135446
1.7729193 0.0091742134
1.7903434 0.0091355582
1.8078528 0.009097558
1.8254474 0.0090601931
1.8431272 0.0090234442
1.8608921 0.0089872929
1.8787423 0.0089517216
1.8966777 0.0089167134
1.9146983 0.0088822517
1.9328041 0.008848321
1.9509951 0.008814906
1.9692713 0.0087819921
1.9876327 0.0087495653
2.0060793 0.0087176119
2.0246111 0.0086861188
2.0432281 0.0086550734
2.0619303 0.0086244634
2.0807178 0.0085942769
2.0995904 0.0085645026
2.1185482 0.0085351294
2.1375913 0.0085061465
2.1567195 0.0084775437
2.1759329 0.0084493108
2.1952316 0.0084214382
2.2146154 0.0083939164
2.2340845 0.0083667364
2.2536387 0.0083398891
2.2732782 0.0083133662
2.2930029 0.0082871592
2.3128127 0.00826126
2.3327078 0.0082356609
2.3526881 0.0082103541
2.3727536 0.0081853323
2.3929042 0.0081605882
2.4131401 0.008136115
2.4334612 0.0081119058
2.4538675 0.0080879539
2.474359 0.008064253
2.4949357 0.0080407967
2.5155976 0.0080175791
2.5363447 0.0079945942
2.557177 0.0079718362
2.5780946 0.0079492995
2.5990973 0.0079269787
2.6201852 0.0079048683
2.6413583 0.0078829633
2.6626167 0.0078612586
2.6839602 0.0078397492
2.7053889 0.0078184303
2.7269029 0.0077972973
2.748502 0.0077763456
2.7701864 0.0077555707
2.7919559 0.0077349682
2.8138107 0.007714534
2.8357506 0.0076942639
2.8577758 0.0076741538
2.8798862 0.0076541998
2.9020817 0.007634398
2.9243625 0.0076147448
2.9467285 0.0075952363
2.9691797 0.0075758691
2.9917161 0.0075566396
3.0143377 0.0075375443
3.0370445 0.00751858
3.0598365 0.0074997433
3.0827137 0.0074810311
3.1056761 0.0074624402
3.1287237 0.0074439676
3.1518565 0.0074256102
3.1750745 0.0074073652
3.1983777 0.0073892297
3.2217662 0.0073712008
3.2452398 0.0073532759
3.2687986 0.0073354523
3.2924427 0.0073177272
3.3161719 0.0073000983
3.3399863 0.0072825628
3.363886 0.0072651185
3.3878708 0.0072477628
3.4119409 0.0072304935
3.4360961 0.0072133081
3.4603366 0.0071962045
3.4846623 0.0071791804
3.5090731 0.0071622337
3.5335692 0.0071453621
3.5581505 0.0071285637
3.582817 0.0071118363
3.6075687 0.0070951781
3.6324055 0.007078587
3.6573276 0.007062061
3.6823349 0.0070455984
3.7074274 0.0070291972
3.7326051 0.0070128557
3.757868 0.006996572
3.7832162 0.0069803445
3.8086495 0.0069641714
3.834168 0.006948051
3.8597717 0.0069319817
3.8854606 0.006915962
3.9112348 0.0068999901
3.9370941 0.0068840646
3.9630386 0.0068681839
3.9890684 0.0068523466
4.0151833 0.0068365511
4.0413835 0.0068207961
4.0676688 0.0068050801
4.0940394 0.0067894018
4.1204951 0.0067737598
4.1470361 0.0067581527
4.1736623 0.0067425793
4.2003736 0.0067270383
4.2271702 0.0067115284
4.254052 0.0066960484
4.281019 0.006680597
4.3080711 0.0066651732
4.3352085 0.0066497756
4.3624311 0.0066344033
4.3897389 0.006619055
4.4171319 0.0066037296
4.4446101 0.0065884261
4.4721735 0.0065731433
4.4998221 0.0065578804
4.527556 0.0065426361
4.555375 0.0065274096
4.5832792 0.0065121999
4.6112686 0.0064970059
4.6393433 0.0064818267
4.6675031 0.0064666614
4.6957481 0.0064515091
4.7240784 0.0064363689
4.7524938 0.0064212398
4.7809945 0.0064061211
4.8095803 0.0063910118
4.8382514 0.0063759112
4.8670076 0.0063608185
4.8958491 0.0063457327
4.9247758 0.0063306532
4.9537876 0.0063155792
4.9828847 0.0063005098
5.012067 0.0062854445
5.0413345 0.0062703823
5.0706872 0.0062553227
5.1001251 0.0062402649
5.1296481 0.0062252082
5.1592564 0.006210152
5.1889499 0.0061950956
5.2187286 0.0061800384
5.2485926 0.0061649796
5.2785417 0.0061499188
5.308576 0.0061348552
5.3386955 0.0061197883
5.3689002 0.0061047175
5.3991902 0.0060896422
5.4295653 0.0060745619
5.4600256 0.006059476
5.4905712 0.0060443839
5.5212019 0.0060292853
5.5519178 0.0060141794
5.582719 0.0059990658
5.6136053 0.0059839441
5.6445769 0.0059688137
5.6756337 0.0059536742
5.7067756 0.0059385251
5.7380028 0.005923366
5.7693152 0.0059081963
5.8007127 0.0058930158
5.8321955 0.0058778238
5.8637635 0.0058626202
5.8954167 0.0058474044
5.9271551 0.005832176
5.9589787 0.0058169347
5.9908875 0.0058016801
6.0228815 0.0057864118
6.0549607 0.0057711295
6.0871251 0.0057558329
6.1193747 0.0057405215
6.1517095 0.0057251951
6.1841295 0.0057098533
6.2166348 0.0056944959
6.2492252 0.0056791225
6.2819008 0.0056637329
6.3146617 0.0056483267
6.3475077 0.0056329037
6.3804389 0.0056174636
6.4134554 0.0056020062
6.446557 0.0055865312
6.4797439 0.0055710384
6.513016 0.0055555275
6.5463732 0.0055399983
6.5798157 0.0055244506
6.6133433 0.0055088842
6.6469562 0.0054932989
6.6806543 0.0054776945
6.7144376 0.0054620708
6.7483061 0.0054464276
6.7822597 0.0054307647
6.8162986 0.0054150821
&
@target G0.S3
@type xy
4.2601867e-05 1.5195407e-10
0.00017040747 2.4330131e-09
0.0003834168 1.2331898e-08
0.00068162986 3.9040363e-08
0.0010650467 9.5519463e-08
0.0015336672 1.9859317e-07
0.0020874915 3.6907026e-07
0.0027265195 6.3189554e-07
0.0034507512 1.0163319e-06
0.0042601867 1.5561751e-06
0.0051548258 2.2900026e-06
0.0061346688 3.2614602e-06
0.0071997154 4.5195874e-06
0.0083499658 6.1191871e-06
0.00958542 8.1212406e-06
0.010906078 1.0593374e-05
0.012311939 1.361038e-05
0.013803005 1.7254801e-05
0.015379274 2.161758e-05
0.017040747 2.6798779e-05
0.018787423 3.2908393e-05
0.020619303 4.0067235e-05
0.022536387 4.8407941e-05
0.024538675 5.807607e-05
0.026626167 6.9231337e-05
0.028798862 8.2048986e-05
0.031056761 9.6721305e-05
0.033399863 0.00011345933
0.03582817 0.00013249473
0.03834168 0.00015408191
0.040940394 0.00017850037
0.043624311 0.00020605733
0.046393433 0.00023709063
0.049247758 0.00027197205
0.052187286 0.00031111096
0.055212019 0.00035495843
0.058321955 0.00040401187
0.061517095 0.00045882018
0.064797439 0.0005199896
0.068162986 0.00058819027
0.071613738 0.00066416363
0.075149693 0.00074873077
0.078770851 0.00084280185
0.082477214 0.00094738677
0.08626878 0.0010636073
0.09014555 0.0011927107
0.094107523 0.0013360854
0.0981547 0.0014952786
0.10228708 0.0016720167
0.10650467 0.0018682281
0.11080745 0.0020860693
0.11519545 0.0023279555
0.11966864 0.0025965948
0.12422704 0.0028950275
0.12887065 0.003226672
0.13359945 0.0035953767
0.13841346 0.0040054804
0.14331268 0.0044618818
0.1482971 0.0049701199
0.15336672 0.0055364668
0.15852155 0.0061680355
0.16376157 0.0068729051
0.16908681 0.0076602659
0.17449725 0.0085405881
0.17999289 0.0095258191
0.18557373 0.010629612
0.19123978 0.011867594
0.19699103 0.013257676
0.20282749 0.01482042
0.20874915 0.016579462
0.21475601 0.018562008
0.22084808 0.020799411
0.22702535 0.023327847
0.23328782 0.02618909
0.2396355 0.029431421
0.24606838 0.033110666
0.25258647 0.03729139
0.25918976 0.042048247
0.26587825 0.047467502
0.27265195 0.05364871
0.27951085 0.060706526
0.28645495 0.068772607
0.29348426 0.077997493
0.30059877 0.088552334
0.30779849 0.10063019
0.3150834 0.11444657
0.32245353 0.13023862
0.32990885 0.14826229
0.33744938 0.16878637
0.34507512 0.19208214
0.35278606 0.21840698
0.3605822 0.24798024
0.36846354 0.28094938
0.37643009 0.31734536
0.38448185 0.35702722
0.3926188 0.39961817
0.40084096 0.44443959
0.40914833 0.49045401
0.41754089 0.53623338
0.42601867 0.57997318
0.43458164 0.61957158
0.44322982 0.65278551
0.4519632 0.67745822
0.46078179 0.69178973
0.46968558 0.69459984
0.47867457 0.68552255
0.48774877 0.66507993
0.49690817 0.63461306
0.50615278 0.59608618
0.51548258 0.55181343
0.5248976 0.50417201
0.53439781 0.45535808
0.54398323 0.40721969
0.55365386 0.36117501
0.56340968 0.31820413
0.57325072 0.27889219
0.58317695 0.24350022
0.59318839 0.21204446
0.60328503 0.18437095
0.61346688 0.1602187
0.62373393 0.13926888
0.63408618 0.12118061
0.64452364 0.10561529
0.6550463 0.092251828
0.66565416 0.08079531
0.67634723 0.07098085
0.6871255 0.062574447
0.69798898 0.055371874
0.70893766 0.049196502
0.71997154 0.043896585
0.73109063 0.039342395
0.74229492 0.035423413
0.75358442 0.03204571
0.76495911 0.029129579
0.77641902 0.026607439
0.78796412 0.024422006
0.79959443 0.022524714
0.81130995 0.020874369
0.82311066 0.019436001
0.83499658 0.018179894
0.84696771 0.017080764
0.85902404 0.016117069
0.87116557 0.015270431
0.8833923 0.014525143
0.89570424 0.013867763
0.90810139 0.013286764
0.92058373 0.012772249
0.93315128 0.012315703
0.94580404 0.011909787
0.958542 0.011548169
0.97136516 0.011225371
0.98427352 0.010936649
0.99726709 0.010677887
1.0103459 0.010445507
1.0235098 0.010236395
1.036759 0.010047837
1.0500934 0.0098774614
1.063513 0.0097231939
1.0770178 0.009583218
1.0906078 0.0094559396
1.104283 0.0093399582
1.1180434 0.0092340417
1.131889 0.0091371041
1.1458198 0.0090481874
1.1598358 0.0089664449
1.173937 0.0088911277
1.1881235 0.0088215723
1.2023951 0.00875719
1.2167519 0.0086974581
1.2311939 0.0086419117
1.2457212 0.008590137
1.2603336 0.0085417651
1.2750313 0.0084964669
1.2898141 0.0084539481
1.3046822 0.0084139458
1.3196354 0.0083762244
1.3346739 0.008340573
1.3497975 0.008306802
1.3650064 0.0082747414
1.3803005 0.0082442383
1.3956797 0.0082151549
1.4111442 0.0081873673
1.4266939 0.0081607637
1.4423288 0.0081352431
1.4580489 0.0081107144
1.4738542 0.008087095
1.4897447 0.0080643103
1.5057204 0.0080422927
1.5217813 0.0080209808
1.5379274 0.0080003191
1.5541587 0.0079802568
1.5704752 0.0079607481
1.5868769 0.007941751
1.6033638 0.0079232274
1.619936 0.0079051425
1.6365933 0.0078874647
1.6533358 0.0078701648
1.6701636 0.0078532165
1.6870765 0.0078365954
1.7040747 0.0078202793
1.721158 0.0078042479
1.7383266 0.0077884824
1.7555803 0.0077729656
1.7729193 0.0077576819
1.7903434 0.0077426165
1.8078528 0.0077277562
1.8254474 0.0077130885
1.8431272 0.0076986021
1.8608921 0.0076842864
1.8787423 0.0076701316
1.8966777 0.0076561287
1.9146983 0.0076422693
1.9328041 0.0076285456
1.9509951 0.0076149504
1.9692713 0.007601477
1.9876327 0.007588119
2.0060793 0.0075748707
2.0246111 0.0075617265
2.0432281 0.0075486814
2.0619303 0.0075357305
2.0807178 0.0075228693
2.0995904 0.0075100937
2.1185482 0.0074973998
2.1375913 0.0074847836
2.1567195 0.0074722419
2.1759329 0.0074597711
2.1952316 0.0074473683
2.2146154 0.0074350304
2.2340845 0.0074227546
2.2536387 0.0074105382
2.2732782 0.0073983788
2.2930029 0.0073862739
2.3128127 0.0073742211
2.3327078 0.0073622184
2.3526881 0.0073502636
2.3727536 0.0073383548
2.3929042 0.0073264899
2.4131401 0.0073146671
2.4334612 0.0073028848
2.4538675 0.0072911411
2.474359 0.0072794345
2.4949357 0.0072677633
2.5155976 0.0072561261
2.5363447 0.0072445214
2.557177 0.0072329477
2.5780946 0.0072214037
2.5990973 0.0072098881
2.6201852 0.0071983995
2.6413583 0.0071869367
2.6626167 0.0071754985
2.6839602 0.0071640837
2.7053889 0.0071526911
2.7269029 0.0071413197
2.748502 0.0071299683
2.7701864 0.0071186358
2.7919559 0.0071073212
2.8138107 0.0070960236
2.8357506 0.0070847418
2.8577758 0.0070734749
2.8798862 0.007062222
2.9020817 0.0070509821
2.9243625 0.0070397543
2.9467285 0.0070285377
2.9691797 0.0070173315
2.9917161 0.0070061347
3.0143377 0.0069949465
3.0370445 0.0069837662
3.0598365 0.0069725927
3.0827137 0.0069614255
3.1056761 0.0069502636
3.1287237 0.0069391063
3.1518565 0.0069279528
3.1750745 0.0069168024
3.1983777 0.0069056543
3.2217662 0.0068945078
3.2452398 0.0068833622
3.2687986 0.0068722168
3.2924427 0.0068610708
3.3161719 0.0068499237
3.3399863 0.0068387747
3.363886 0.0068276231
3.3878708 0.0068164683
3.4119409 0.0068053096
3.4360961 0.0067941465
3.4603366 0.0067829782
3.4846623 0.0067718042
3.5090731 0.0067606238
3.5335692 0.0067494365
3.5581505 0.0067382416
3.582817 0.0067270386
3.6075687 0.0067158268
3.6324055 0.0067046058
3.6573276 0.0066933749
3.6823349 0.0066821336
3.7074274 0.0066708813
3.7326051 0.0066596175
3.757868 0.0066483416
3.7832162 0.0066370533
3.8086495 0.0066257518
3.834168 0.0066144367
3.8597717 0.0066031075
3.8854606 0.0065917637
3.9112348 0.0065804048
3.9370941 0.0065690303
3.9630386 0.0065576398
3.9890684 0.0065462327
4.0151833 0.0065348087
4.0413835 0.0065233671
4.0676688 0.0065119077
4.0940394 0.0065004299
4.1204951 0.0064889332
4.1470361 0.0064774174
4.1736623 0.0064658819
4.2003736 0.0064543262
4.2271702 0.0064427501
4.254052 0.0064311531
4.281019 0.0064195347
4.3080711 0.0064078946
4.3352085 0.0063962324
4.3624311 0.0063845477
4.3897389 0.0063728401
4.4171319 0.0063611093
4.4446101 0.0063493548
4.4721735 0.0063375764
4.4998221 0.0063257735
4.527556 0.006313946
4.555375 0.0063020934
4.5832792 0.0062902155
4.6112686 0.0062783118
4.6393433 0.006266382
4.6675031 0.0062544259
4.6957481 0.006242443
4.7240784 0.0062304331
4.7524938 0.0062183959
4.7809945 0.0062063311
4.8095803 0.0061942383
4.8382514 0.0061821173
4.8670076 0.0061699677
4.8958491 0.0061577894
4.9247758 0.006145582
4.9537876 0.0061333452
4.9828847 0.0061210789
5.012067 0.0061087826
5.0413345 0.0060964563
5.0706872 0.0060840995
5.1001251 0.0060717121
5.1296481 0.0060592938
5.1592564 0.0060468445
5.1889499 0.0060343638
5.2187286 0.0060218515
5.2485926 0.0060093074
5.2785417 0.0059967314
5.308576 0.0059841231
5.3386955 0.0059714824
5.3689002 0.0059588091
5.3991902 0.005946103
5.4295653 0.0059333639
5.4600256 0.0059205916
5.4905712 0.0059077859
5.5212019 0.0058949467
5.5519178 0.0058820737
5.582719 0.0058691669
5.6136053 0.0058562261
5.6445769 0.005843251
5.6756337 0.0058302416
5.7067756 0.0058171977
5.7380028 0.0058041192
5.7693152 0.005791006
5.8007127 0.0057778578
5.8321955 0.0057646746
5.8637635 0.0057514562
5.8954167 0.0057382026
5.9271551 0.0057249136
5.9589787 0.0057115892
5.9908875 0.0056982291
6.0228815 0.0056848334
6.0549607 0.0056714019
6.0871251 0.0056579346
6.1193747 0.0056444313
6.1517095 0.0056308921
6.1841295 0.0056173167
6.2166348 0.0056037052
6.2492252 0.0055900575
6.2819008 0.0055763735
6.3146617 0.0055626531
6.3475077 0.0055488964
6.3804389 0.0055351033
6.4134554 0.0055212738
6.446557 0.0055074077
6.4797439 0.0054935051
6.513016 0.005479566
6.5463732 0.0054655904
6.5798157 0.0054515782
6.6133433 0.0054375294
6.6469562 0.005423444
6.6806543 0.005409322
6.7144376 0.0053951634
6.7483061 0.0053809683
6.7822597 0.0053667366
6.8162986 0.0053524684
&
@target G0.S4
@type xy
4.2601867e-05 3.0841762e-10
0.00017040747 4.9386571e-09
0.0003834168 2.5035541e-08
0.00068162986 7.9273614e-08
0.0010650467 1.9400796e-07
0.0015336672 4.0348747e-07
0.0020874915 7.5013271e-07
0.0027265195 1.2848812e-06
0.0034507512 2.0676037e-06
0.0042601867 3.1675958e-06
0.0051548258 4.6641493e-06
0.0061346688 6.6472106e-06
0.0071997154 9.2181322e-06
0.0083499658 1.2490524e-05
0.00958542 1.6591218e-05
0.010906078 2.166135e-05
0.012311939 2.7857575e-05
0.013803005 3.5353431e-05
0.015379274 4.4340865e-05
0.017040747 5.503193e-05
0.018787423 6.7660689e-05
0.020619303 8.2485339e-05
0.022536387 9.9790577e-05
0.024538675 0.00011989024
0.026626167 0.00014313027
0.028798862 0.00016989199
0.031056761 0.00020059579
0.033399863 0.00023570527
0.03582817 0.00027573178
0.03834168 0.00032123965
0.040940394 0.00037285193
0.043624311 0.00043125683
0.046393433 0.00049721506
0.049247758 0.00057156793
0.052187286 0.00065524657
0.055212019 0.00074928227
0.058321955 0.00085481812
0.061517095 0.00097312214
0.064797439 0.0011056022
0.068162986 0.0012538227
0.071613738 0.0014195238
0.075149693 0.0016046427
0.078770851 0.0018113386
0.082477214 0.00204202
0.08626878 0.0022993767
0.09014555 0.0025864161
0.094107523 0.0029065043
0.0981547 0.003263413
0.10228708 0.0036613742
0.10650467 0.0041051415
0.11080745 0.0046000617
0.11519545 0.0051521563
0.11966864 0.0057682159
0.12422704 0.0064559091
0.12887065 0.0072239076
0.13359945 0.0080820323
0.13841346 0.0090414212
0.14331268 0.010114725
0.1482971 0.011316336
0.15336672 0.01266265
0.15852155 0.014172379
0.16376157 0.015866907
0.16908681 0.017770716
0.17449725 0.019911881
0.17999289 0.022322642
0.18557373 0.025040094
0.19123978 0.028106978
0.19699103 0.031572624
0.20282749 0.035494058
0.20874915 0.039937302
0.21475601 0.044978909
0.22084808 0.050707764
0.22702535 0.05722721
0.23328782 0.064657535
0.2396355 0.073138891
0.24606838 0.082834704
0.25258647 0.093935632
0.25918976 0.10666414
0.26587825 0.12127975
0.27265195 0.13808497
0.27951085 0.15743187
0.28645495 0.17972936
0.29348426 0.20545069
0.30059877 0.23514108
0.30779849 0.26942468
0.3150834 0.3090098
0.32245353 0.35469098
0.32990885 0.40734552
0.33744938 0.4679213
0.34507512 0.53741165
0.35278606 0.61681178
0.3605822 0.70705019
0.36846354 0.80888834
0.37643009 0.92278231
0.38448185 1.0487038
0.3926188 1.1859245
0.40084096 1.3327794
0.40914833 1.4864418
0.41754089 1.6427604
0.42601867 1.7962267
0.43458164 1.9401456
0.44322982 2.0670613
0.4519632 2.1694433
0.46078179 2.2405627
0.46968558 2.2754071
0.47867457 2.2714349
0.48774877 2.2289788
0.49690817 2.1511912
0.50615278 2.0435449
0.51548258 1.9130239
0.5248976 1.767201
0.53439781 1.6133962
0.54398323 1.4580485
0.55365386 1.3063523
0.56340968 1.1621404
0.57325072 1.0279533
0.58317695 0.90522064
0.59318839 0.79449333
0.60328503 0.69567612
0.61346688 0.60823525
0.62373393 0.53136755
0.63408618 0.46412913
0.64452364 0.40552752
0.6550463 0.35458365
0.66565416 0.31037046
0.67634723 0.27203465
0.6871255 0.23880642
0.69798898 0.21000149
0.70893766 0.18501819
0.71997154 0.16333169
0.73109063 0.14448697
0.74229492 0.12809116
0.75358442 0.11380615
0.76495911 0.10134149
0.77641902 0.090448052
0.78796412 0.080912229
0.79959443 0.072550928
0.81130995 0.065207157
0.82311066 0.058746225
0.83499658 0.053052474
0.84696771 0.048026484
0.85902404 0.043582691
0.87116557 0.03964735
0.8833923 0.036156818
0.89570424 0.033056078
0.90810139 0.0302975
0.92058373 0.027839779
0.93315128 0.025647037
0.94580404 0.023688057
0.958542 0.021935634
0.97136516 0.020366017
0.98427352 0.018958437
0.99726709 0.017694703
1.0103459 0.016558854
1.0235098 0.015536868
1.036759 0.014616399
1.0500934 0.013786566
1.063513 0.013037761
1.0770178 0.012361491
1.0906078 0.011750232
1.104283 0.011197312
1.1180434 0.010696806
1.131889 0.010243445
1.1458198 0.0098325369
1.1598358 0.0094598963
1.173937 0.009121787
1.1881235 0.0088148684
1.2023951 0.0085361502
1.2167519 0.0082829525
1.2311939 0.0080528706
1.2457212 0.0078437444
1.2603336 0.0076536311
1.2750313 0.0074807817
1.2898141 0.0073236199
1.3046822 0.0071807235
1.3196354 0.0070508083
1.3346739 0.006932713
1.3497975 0.0068253873
1.3650064 0.0067278795
1.3803005 0.006639327
1.3956797 0.0065589474
1.4111442 0.0064860299
1.4266939 0.0064199287
1.4423288 0.0063600562
1.4580489 0.0063058777
1.4738542 0.0062569061
1.4897447 0.0062126973
1.5057204 0.0061728461
1.5217813 0.0061369826
1.5379274 0.0061047689
1.5541587 0.0060758963
1.5704752 0.0060500821
1.5868769 0.0060270679
1.6033638 0.0060066167
1.619936 0.0059885117
1.6365933 0.005972554
1.6533358 0.005958561
1.6701636 0.0059463654
1.6870765 0.0059358134
1.7040747 0.0059267638
1.721158 0.0059190868
1.7383266 0.0059126631
1.7555803 0.005907383
1.7729193 0.0059031455
1.7903434 0.0058998577
1.8078528 0.005897434
1.8254474 0.0058957956
1.8431272 0.0058948699
1.8608921 0.00589459
1.8787423 0.0058948943
1.8966777 0.0058957259
1.9146983 0.0058970323
1.9328041 0.0058987653
1.9509951 0.0059008802
1.9692713 0.0059033358
1.9876327 0.0059060943
2.0060793 0.0059091205
2.0246111 0.0059123821
2.0432281 0.0059158493
2.0619303 0.0059194945
2.0807178 0.0059232924
2.0995904 0.0059272194
2.1185482 0.0059312541
2.1375913 0.0059353763
2.1567195 0.0059395676
2.1759329 0.0059438112
2.1952316 0.0059480914
2.2146154 0.0059523936
2.2340845 0.0059567047
2.2536387 0.0059610124
2.2732782 0.0059653054
2.2930029 0.0059695733
2.3128127 0.0059738066
2.3327078 0.0059779965
2.3526881 0.005982135
2.3727536 0.0059862147
2.3929042 0.0059902287
2.4131401 0.005994171
2.4334612 0.0059980358
2.4538675 0.0060018178
2.474359 0.0060055125
2.4949357 0.0060091153
2.5155976 0.0060126225
2.5363447 0.0060160304
2.557177 0.0060193359
2.5780946 0.0060225358
2.5990973 0.0060256277
2.6201852 0.0060286092
2.6413583 0.006031478
2.6626167 0.0060342324
2.6839602 0.0060368706
2.7053889 0.006039391
2.7269029 0.0060417925
2.748502 0.0060440738
2.7701864 0.006046234
2.7919559 0.0060482722
2.8138107 0.0060501877
2.8357506 0.0060519798
2.8577758 0.0060536481
2.8798862 0.0060551923
2.9020817 0.006056612
2.9243625 0.006057907
2.9467285 0.0060590772
2.9691797 0.0060601226
2.9917161 0.0060610432
3.0143377 0.0060618391
3.0370445 0.0060625105
3.0598365 0.0060630575
3.0827137 0.0060634803
3.1056761 0.0060637794
3.1287237 0.006063955
3.1518565 0.0060640075
3.1750745 0.0060639372
3.1983777 0.0060637447
3.2217662 0.0060634304
3.2452398 0.0060629948
3.2687986 0.0060624383
3.2924427 0.0060617616
3.3161719 0.0060609651
3.3399863 0.0060600494
3.363886 0.0060590151
3.3878708 0.0060578628
3.4119409 0.0060565931
3.4360961 0.0060552065
3.4603366 0.0060537037
3.4846623 0.0060520853
3.5090731 0.006050352
3.5335692 0.0060485043
3.5581505 0.0060465429
3.582817 0.0060444684
3.6075687 0.0060422815
3.6324055 0.0060399828
3.6573276 0.0060375728
3.6823349 0.0060350524
3.7074274 0.006032422
3.7326051 0.0060296823
3.757868 0.0060268339
3.7832162 0.0060238776
3.8086495 0.0060208138
3.834168 0.0060176432
3.8597717 0.0060143664
3.8854606 0.006010984
3.9112348 0.0060074967
3.9370941 0.0060039049
3.9630386 0.0060002094
3.9890684 0.0059964107
4.0151833 0.0059925094
4.0413835 0.005988506
4.0676688 0.0059844011
4.0940394 0.0059801953
4.1204951 0.0059758892
4.1470361 0.0059714833
4.1736623 0.0059669782
4.2003736 0.0059623743
4.2271702 0.0059576722
4.254052 0.0059528725
4.281019 0.0059479757
4.3080711 0.0059429823
4.3352085 0.0059378927
4.3624311 0.0059327076
4.3897389 0.0059274274
4.4171319 0.0059220526
4.4446101 0.0059165836
4.4721735 0.005911021
4.4998221 0.0059053653
4.527556 0.0058996168
4.555375 0.0058937762
4.5832792 0.0058878437
4.6112686 0.0058818199
4.6393433 0.0058757053
4.6675031 0.0058695002
4.6957481 0.0058632051
4.7240784 0.0058568204
4.7524938 0.0058503466
4.7809945 0.0058437841
4.8095803 0.0058371332
4.8382514 0.0058303945
4.8670076 0.0058235682
4.8958491 0.0058166549
4.9247758 0.0058096549
4.9537876 0.0058025686
4.9828847 0.0057953964
5.012067 0.0057881386
5.0413345 0.0057807957
5.0706872 0.005773368
5.1001251 0.005765856
5.1296481 0.0057582599
5.1592564 0.0057505801
5.1889499 0.0057428171
5.2187286 0.0057349711
5.2485926 0.0057270425
5.2785417 0.0057190318
5.308576 0.0057109391
5.3386955 0.0057027649
5.3689002 0.0056945095
5.3991902 0.0056861732
5.4295653 0.0056777565
5.4600256 0.0056692595
5.4905712 0.0056606828
5.5212019 0.0056520265
5.5519178 0.005643291
5.582719 0.0056344767
5.6136053 0.0056255839
5.6445769 0.0056166128
5.6756337 0.0056075639
5.7067756 0.0055984374
5.7380028 0.0055892337
5.7693152 0.005579953
5.8007127 0.0055705958
5.8321955 0.0055611622
5.8637635 0.0055516527
5.8954167 0.0055420674
5.9271551 0.0055324069
5.9589787 0.0055226712
5.9908875 0.0055128608
6.0228815 0.005502976
6.0549607 0.0054930171
6.0871251 0.0054829843
6.1193747 0.005472878
6.1517095 0.0054626986
6.1841295 0.0054524462
6.2166348 0.0054421212
6.2492252 0.0054317239
6.2819008 0.0054212546
6.3146617 0.0054107137
6.3475077 0.0054001014
6.3804389 0.005389418
6.4134554 0.0053786638
6.446557 0.0053678392
6.4797439 0.0053569444
6.513016 0.0053459797
6.5463732 0.0053349456
6.5798157 0.0053238422
6.6133433 0.0053126698
6.6469562 0.0053014289
6.6806543 0.0052901196
6.7144376 0.0052787423
6.7483061 0.0052672974
6.7822597 0.005255785
6.8162986 0.0052442056
&


==> plot_more <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 0
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Aug 30 19:16:07 2021"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, -0.9, 9, 2
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.550000, 0.625703, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label ""
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 1
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\si\N\h{-0.2}\SLO\N+E\si\N\h{-0.2}\SNLO\N [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.5
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.85, 0.4
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 1
@    s0 symbol size 0.500000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 1
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 2
@    s0 line linewidth 1.5
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/mares/jerry/test_per/e_150450_w1_clo-25_dlo0_cnlo-59_dlo0"
@    s0 legend  "h\v{0.65}\h{-0.5}\z{0.6}_ \N\xw\0=1 MeV"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 0.500000
@    s2 symbol color 3
@    s2 symbol pattern 1
@    s2 symbol fill color 3
@    s2 symbol fill pattern 3
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 2
@    s2 line linewidth 1.5
@    s2 line color 3
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 3
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/mares/jerry/test_per/e_150450_w4_clo-25_dlo0_cnlo-59_dlo0"
@    s2 legend  "h\v{0.65}\h{-0.5}\z{0.6}_ \N\xw\0=4 MeV"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 4
@    s3 symbol size 0.500000
@    s3 symbol color 4
@    s3 symbol pattern 1
@    s3 symbol fill color 4
@    s3 symbol fill pattern 4
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 1
@    s3 line linestyle 2
@    s3 line linewidth 1.5
@    s3 line color 4
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 4
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "/home/mares/jerry/test_per/e_150450_w10_clo-25_dlo0_cnlo-59_dlo0"
@    s3 legend  "\h\v{0.65}\h{-0.5}\z{0.6}_ \N\xw\0=10 MeV"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 6
@    s4 symbol size 0.500000
@    s4 symbol color 2
@    s4 symbol pattern 1
@    s4 symbol fill color 2
@    s4 symbol fill pattern 6
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 1
@    s4 line linestyle 2
@    s4 line linewidth 1.5
@    s4 line color 2
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 2
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "/home/mares/jerry/test_per/e_150450_w20_clo-25_dlo0_cnlo-59_dlo0"
@    s4 legend  "h\v{0.65}\h{-0.5}\z{0.6}_ \N\xw\0=20 MeV"
@g1 on
@g1 hidden false
@g1 type XY
@g1 stacked false
@g1 bar hgap 0.000000
@g1 fixedpoint off
@g1 fixedpoint type 0
@g1 fixedpoint xy 0.000000, 0.000000
@g1 fixedpoint format general general
@g1 fixedpoint prec 6, 6
@with g1
@    world 0, 0, 1, 1
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.768414, 0.550000, 1.244118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "T\slab\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\xs\0(\S3\NP\s0\N) [MeV\S-2\N]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@g2 on
@g2 hidden false
@g2 type XY
@g2 stacked false
@g2 bar hgap 0.000000
@g2 fixedpoint off
@g2 fixedpoint type 0
@g2 fixedpoint xy 0.000000, 0.000000
@g2 fixedpoint format general general
@g2 fixedpoint prec 6, 6
@with g2
@    world 0, 0, 1, 1
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 0.625703, 0.550000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "i"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "E\si\N\h{-0.2}\SNLO\N [MeV]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@g3 on
@g3 hidden false
@g3 type XY
@g3 stacked false
@g3 bar hgap 0.000000
@g3 fixedpoint off
@g3 fixedpoint type 0
@g3 fixedpoint xy 0.000000, 0.000000
@g3 fixedpoint format general general
@g3 fixedpoint prec 6, 6
@with g3
@    world 0, 0, 1, 1
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.768414, 0.150000, 1.244118, 0.550000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 0
@    xaxis  bar linestyle 0
@    xaxis  bar linewidth 1.0
@    xaxis  label ""
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.000000
@    xaxis  label font 0
@    xaxis  label color 0
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 0
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 0
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.000000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 0
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar off
@    yaxis  bar color 0
@    yaxis  bar linestyle 0
@    yaxis  bar linewidth 1.0
@    yaxis  label ""
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.000000
@    yaxis  label font 0
@    yaxis  label color 0
@    yaxis  label place normal
@    yaxis  tick off
@    yaxis  tick major 0.2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 0
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 0
@    yaxis  tick major grid off
@    yaxis  tick minor color 0
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 0
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel off
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.000000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 0
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 0
@    frame pattern 0
@    frame background color 0
@    frame background pattern 0
@target G0.S0
@type xy
1 0.016519928
2 0.048456722
3 0.095056343
4 0.15315685
5 0.21293185
6 0.24356822
7 0.19769663
8 0.20525836
9 0.39659412
10 0.61733288
11 0.82362475
12 1.0286538
13 1.2415897
14 1.4667043
15 1.7060448
16 1.9606792
17 2.2312148
&
@target G0.S2
@type xy
1 0.14676438
2 -0.13878615
3 0.18537767
4 1.048305
5 1.9416157
6 3.0072538
7 4.2760379
8 5.758532
9 7.4608681
&
@target G0.S3
@type xy
1 -0.092035965
2 -0.058685258
3 1.405945
4 3.126186
5 5.371435
6 8.1942894
7 11.616758
8 15.646232
9 20.269103
&
@target G0.S4
@type xy
1 -0.49671569
2 0.76261171
3 3.2923537
4 6.9212185
5 11.84029
6 18.079751
7 25.511619
8 33.818252
&


==> rev_cross <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Sep 13 18:09:47 2021"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, 0, 7, 0.008
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.180000, 0.150000, 0.663262, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "E\scm\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 1
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\xs\0(\S3\NP\s0\N) [MeV\S-2\N]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 0.001
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.28, 0.6
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.500000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 2
@    s0 symbol pattern 1
@    s0 symbol fill color 2
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 3
@    s0 line linewidth 2.0
@    s0 line color 2
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 2
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/chiehjen/jerry/test_per/709per"
@    s0 legend  "LO"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 2.0
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "Cols 1:3"
@    s1 legend  "LO+NLO\sper"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 0
@    s2 symbol size 1.000000
@    s2 symbol color 4
@    s2 symbol pattern 1
@    s2 symbol fill color 4
@    s2 symbol fill pattern 0
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 1
@    s2 line linestyle 2
@    s2 line linewidth 4.5
@    s2 line color 4
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 4
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/chiehjen/jerry/test_per/709non"
@    s2 legend  "LO+NLO\snon-per"
@g1 on
@g1 hidden false
@g1 type XY
@g1 stacked false
@g1 bar hgap 0.000000
@g1 fixedpoint off
@g1 fixedpoint type 0
@g1 fixedpoint xy 0.000000, 0.000000
@g1 fixedpoint format general general
@g1 fixedpoint prec 6, 6
@with g1
@    world 0, 0, 0.005, 13
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.746791, 0.150000, 1.244118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "E\scm\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 0.002
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label ""
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 2
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.5, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 4
@    s1 symbol pattern 1
@    s1 symbol fill color 4
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 2
@    s1 line linewidth 4.5
@    s1 line color 4
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 4
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/chiehjen/jerry/test_per/fort.709"
@    s1 legend  ""
@target G0.S0
@type xy
4.2601867e-05 4.9714097e-10
0.00017040747 7.9416564e-09
0.0003834168 4.0098671e-08
0.00068162986 1.2626498e-07
0.0010650467 3.0680869e-07
0.0015336672 6.3253909e-07
0.0020874915 1.1639204e-06
0.0027265195 1.9701463e-06
0.0034507512 3.1280953e-06
0.0042601867 4.7211879e-06
0.0051548258 6.8381691e-06
0.0061346688 9.5718403e-06
0.0071997154 1.3017764e-05
0.0083499658 1.7272966e-05
0.00958542 2.2434655e-05
0.010906078 2.8598985e-05
0.012311939 3.5859877e-05
0.013803005 4.4307912e-05
0.015379274 5.4029318e-05
0.017040747 6.5105059e-05
0.018787423 7.7610034e-05
0.020619303 9.1612384e-05
0.022536387 0.00010717293
0.024538675 0.00012434473
0.026626167 0.00014317274
0.028798862 0.00016369358
0.031056761 0.0001859355
0.033399863 0.00020991828
0.03582817 0.00023565341
0.03834168 0.00026314418
0.040940394 0.00029238602
0.043624311 0.00032336678
0.046393433 0.00035606707
0.049247758 0.00039046076
0.052187286 0.00042651537
0.055212019 0.00046419262
0.058321955 0.00050344888
0.061517095 0.00054423572
0.064797439 0.00058650044
0.068162986 0.00063018658
0.071613738 0.00067523444
0.075149693 0.00072158158
0.078770851 0.0007691633
0.082477214 0.00081791311
0.08626878 0.00086776318
0.09014555 0.00091864475
0.094107523 0.00097048851
0.0981547 0.001023225
0.10228708 0.0010767848
0.10650467 0.0011310992
0.11080745 0.0011860999
0.11519545 0.0012417199
0.11966864 0.0012978931
0.12422704 0.0013545551
0.12887065 0.0014116429
0.13359945 0.0014690952
0.13841346 0.0015268526
0.14331268 0.0015848577
0.1482971 0.0016430549
0.15336672 0.001701391
0.15852155 0.0017598147
0.16376157 0.0018182769
0.16908681 0.0018767308
0.17449725 0.0019351316
0.17999289 0.001993437
0.18557373 0.0020516066
0.19123978 0.0021096022
0.19699103 0.0021673877
0.20282749 0.0022249292
0.20874915 0.0022821947
0.21475601 0.0023391542
0.22084808 0.0023957797
0.22702535 0.0024520449
0.23328782 0.0025079257
0.2396355 0.0025633992
0.24606838 0.0026184446
0.25258647 0.0026730425
0.25918976 0.0027271753
0.26587825 0.0027808266
0.27265195 0.0028339817
0.27951085 0.002886627
0.28645495 0.0029387503
0.29348426 0.0029903408
0.30059877 0.0030413887
0.30779849 0.0030918854
0.3150834 0.0031418232
0.32245353 0.0031911956
0.32990885 0.003239997
0.33744938 0.0032882226
0.34507512 0.0033358685
0.35278606 0.0033829317
0.3605822 0.0034294098
0.36846354 0.0034753011
0.37643009 0.0035206047
0.38448185 0.0035653201
0.3926188 0.0036094475
0.40084096 0.0036529878
0.40914833 0.003695942
0.41754089 0.0037383118
0.42601867 0.0037800995
0.43458164 0.0038213074
0.44322982 0.0038619385
0.4519632 0.003901996
0.46078179 0.0039414833
0.46968558 0.0039804044
0.47867457 0.0040187633
0.48774877 0.0040565643
0.49690817 0.004093812
0.50615278 0.004130511
0.51548258 0.0041666663
0.5248976 0.004202283
0.53439781 0.0042373662
0.54398323 0.0042719212
0.55365386 0.0043059537
0.56340968 0.004339469
0.57325072 0.0043724727
0.58317695 0.0044049707
0.59318839 0.0044369687
0.60328503 0.0044684724
0.61346688 0.0044994878
0.62373393 0.0045300206
0.63408618 0.0045600768
0.64452364 0.0045896623
0.6550463 0.0046187831
0.66565416 0.0046474449
0.67634723 0.0046756538
0.6871255 0.0047034156
0.69798898 0.0047307363
0.70893766 0.0047576215
0.71997154 0.0047840773
0.73109063 0.0048101092
0.74229492 0.0048357232
0.75358442 0.0048609248
0.76495911 0.0048857198
0.77641902 0.0049101138
0.78796412 0.0049341122
0.79959443 0.0049577207
0.81130995 0.0049809446
0.82311066 0.0050037893
0.83499658 0.0050262603
0.84696771 0.0050483627
0.85902404 0.0050701018
0.87116557 0.0050914826
0.8833923 0.0051125104
0.89570424 0.00513319
0.90810139 0.0051535265
0.92058373 0.0051735247
0.93315128 0.0051931895
0.94580404 0.0052125255
0.958542 0.0052315375
0.97136516 0.00525023
0.98427352 0.0052686077
0.99726709 0.0052866749
1.0103459 0.0053044361
1.0235098 0.0053218956
1.036759 0.0053390577
1.0500934 0.0053559266
1.063513 0.0053725064
1.0770178 0.0053888012
1.0906078 0.0054048149
1.104283 0.0054205516
1.1180434 0.005436015
1.131889 0.0054512091
1.1458198 0.0054661374
1.1598358 0.0054808037
1.173937 0.0054952116
1.1881235 0.0055093647
1.2023951 0.0055232664
1.2167519 0.0055369202
1.2311939 0.0055503294
1.2457212 0.0055634974
1.2603336 0.0055764273
1.2750313 0.0055891224
1.2898141 0.0056015859
1.3046822 0.0056138207
1.3196354 0.0056258299
1.3346739 0.0056376165
1.3497975 0.0056491833
1.3650064 0.0056605334
1.3803005 0.0056716693
1.3956797 0.005682594
1.4111442 0.0056933101
1.4266939 0.0057038202
1.4423288 0.0057141271
1.4580489 0.0057242331
1.4738542 0.0057341409
1.4897447 0.0057438528
1.5057204 0.0057533714
1.5217813 0.005762699
1.5379274 0.0057718378
1.5541587 0.0057807902
1.5704752 0.0057895585
1.5868769 0.0057981448
1.6033638 0.0058065512
1.619936 0.00581478
1.6365933 0.005822833
1.6533358 0.0058307125
1.6701636 0.0058384204
1.6870765 0.0058459586
1.7040747 0.0058533291
1.721158 0.0058605337
1.7383266 0.0058675743
1.7555803 0.0058744527
1.7729193 0.0058811706
1.7903434 0.0058877299
1.8078528 0.0058941322
1.8254474 0.0059003792
1.8431272 0.0059064726
1.8608921 0.0059124138
1.8787423 0.0059182047
1.8966777 0.0059238465
1.9146983 0.005929341
1.9328041 0.0059346896
1.9509951 0.0059398937
1.9692713 0.0059449548
1.9876327 0.0059498742
2.0060793 0.0059546535
2.0246111 0.0059592938
2.0432281 0.0059637965
2.0619303 0.005968163
2.0807178 0.0059723944
2.0995904 0.0059764921
2.1185482 0.0059804573
2.1375913 0.0059842911
2.1567195 0.0059879948
2.1759329 0.0059915694
2.1952316 0.0059950162
2.2146154 0.0059983362
2.2340845 0.0060015305
2.2536387 0.0060046002
2.2732782 0.0060075463
2.2930029 0.0060103698
2.3128127 0.0060130718
2.3327078 0.0060156532
2.3526881 0.006018115
2.3727536 0.0060204581
2.3929042 0.0060226835
2.4131401 0.0060247921
2.4334612 0.0060267847
2.4538675 0.0060286622
2.474359 0.0060304256
2.4949357 0.0060320755
2.5155976 0.0060336129
2.5363447 0.0060350386
2.557177 0.0060363532
2.5780946 0.0060375577
2.5990973 0.0060386528
2.6201852 0.0060396392
2.6413583 0.0060405176
2.6626167 0.0060412888
2.6839602 0.0060419535
2.7053889 0.0060425122
2.7269029 0.0060429659
2.748502 0.006043315
2.7701864 0.0060435602
2.7919559 0.0060437022
2.8138107 0.0060437415
2.8357506 0.0060436789
2.8577758 0.0060435149
2.8798862 0.00604325
2.9020817 0.0060428849
2.9243625 0.0060424201
2.9467285 0.0060418561
2.9691797 0.0060411936
2.9917161 0.006040433
3.0143377 0.0060395749
3.0370445 0.0060386197
3.0598365 0.0060375681
3.0827137 0.0060364203
3.1056761 0.0060351771
3.1287237 0.0060338387
3.1518565 0.0060324057
3.1750745 0.0060308786
3.1983777 0.0060292577
3.2217662 0.0060275436
3.2452398 0.0060257366
3.2687986 0.0060238371
3.2924427 0.0060218457
3.3161719 0.0060197626
3.3399863 0.0060175883
3.363886 0.0060153232
3.3878708 0.0060129676
3.4119409 0.0060105219
3.4360961 0.0060079866
3.4603366 0.0060053619
3.4846623 0.0060026482
3.5090731 0.0059998459
3.5335692 0.0059969553
3.5581505 0.0059939767
3.582817 0.0059909105
3.6075687 0.005987757
3.6324055 0.0059845165
3.6573276 0.0059811893
3.6823349 0.0059777758
3.7074274 0.0059742761
3.7326051 0.0059706908
3.757868 0.0059670199
3.7832162 0.0059632639
3.8086495 0.0059594229
3.834168 0.0059554973
3.8597717 0.0059514874
3.8854606 0.0059473934
3.9112348 0.0059432156
3.9370941 0.0059389541
3.9630386 0.0059346094
3.9890684 0.0059301817
4.0151833 0.0059256711
4.0413835 0.005921078
4.0676688 0.0059164025
4.0940394 0.005911645
4.1204951 0.0059068056
4.1470361 0.0059018846
4.1736623 0.0058968823
4.2003736 0.0058917987
4.2271702 0.0058866342
4.254052 0.005881389
4.281019 0.0058760633
4.3080711 0.0058706573
4.3352085 0.0058651713
4.3624311 0.0058596053
4.3897389 0.0058539597
4.4171319 0.0058482347
4.4446101 0.0058424303
4.4721735 0.005836547
4.4998221 0.0058305847
4.527556 0.0058245438
4.555375 0.0058184245
4.5832792 0.0058122268
4.6112686 0.0058059511
4.6393433 0.0057995975
4.6675031 0.0057931661
4.6957481 0.0057866573
4.7240784 0.0057800711
4.7524938 0.0057734078
4.7809945 0.0057666675
4.8095803 0.0057598504
4.8382514 0.0057529567
4.8670076 0.0057459866
4.8958491 0.0057389402
4.9247758 0.0057318178
4.9537876 0.0057246195
4.9828847 0.0057173454
5.012067 0.0057099958
5.0413345 0.0057025709
5.0706872 0.0056950708
5.1001251 0.0056874957
5.1296481 0.0056798457
5.1592564 0.0056721211
5.1889499 0.005664322
5.2187286 0.0056564486
5.2485926 0.0056485011
5.2785417 0.0056404796
5.308576 0.0056323843
5.3386955 0.0056242154
5.3689002 0.0056159731
5.3991902 0.0056076575
5.4295653 0.0055992688
5.4600256 0.0055908073
5.4905712 0.005582273
5.5212019 0.0055736661
5.5519178 0.0055649869
5.582719 0.0055562355
5.6136053 0.005547412
5.6445769 0.0055385168
5.6756337 0.0055295499
5.7067756 0.0055205115
5.7380028 0.0055114018
5.7693152 0.005502221
5.8007127 0.0054929693
5.8321955 0.0054836469
5.8637635 0.0054742539
5.8954167 0.0054647905
5.9271551 0.005455257
5.9589787 0.0054456536
5.9908875 0.0054359803
6.0228815 0.0054262374
6.0549607 0.0054164252
6.0871251 0.0054065437
6.1193747 0.0053965933
6.1517095 0.005386574
6.1841295 0.0053764862
6.2166348 0.0053663299
6.2492252 0.0053561055
6.2819008 0.0053458131
6.3146617 0.0053354529
6.3475077 0.0053250251
6.3804389 0.00531453
6.4134554 0.0053039678
6.446557 0.0052933386
6.4797439 0.0052826427
6.513016 0.0052718804
6.5463732 0.0052610517
6.5798157 0.0052501571
6.6133433 0.0052391966
6.6469562 0.0052281705
6.6806543 0.0052170791
6.7144376 0.0052059226
6.7483061 0.0051947012
6.7822597 0.0051834151
6.8162986 0.0051720646
&
@target G0.S1
@type xy
4.2601867e-05 1.9620766e-09
0.00017040747 3.131884e-08
0.0003834168 1.5792676e-07
0.00068162986 4.9637999e-07
0.0010650467 1.2033194e-06
0.0015336672 2.4737812e-06
0.0020874915 4.5366944e-06
0.0027265195 7.649661e-06
0.0034507512 1.2093171e-05
0.0042601867 1.8164412e-05
0.0051548258 2.6170854e-05
0.0061346688 3.6423763e-05
0.0071997154 4.9231818e-05
0.0083499658 6.4894992e-05
0.00958542 8.3698807e-05
0.010906078 0.00010590912
0.012311939 0.00013176748
0.013803005 0.00016148722
0.015379274 0.00019525023
0.017040747 0.00023320448
0.018787423 0.00027546234
0.020619303 0.00032209961
0.022536387 0.00037315528
0.024538675 0.00042863193
0.026626167 0.00048849671
0.028798862 0.00055268291
0.031056761 0.0006210919
0.033399863 0.00069359551
0.03582817 0.00077003867
0.03834168 0.00085024226
0.040940394 0.00093400612
0.043624311 0.0010211121
0.046393433 0.0011113273
0.049247758 0.0012044069
0.052187286 0.0013000971
0.055212019 0.0013981383
0.058321955 0.0014982673
0.061517095 0.00160022
0.064797439 0.0017037338
0.068162986 0.0018085492
0.071613738 0.0019144123
0.075149693 0.0020210756
0.078770851 0.0021282999
0.082477214 0.0022358555
0.08626878 0.0023435228
0.09014555 0.0024510932
0.094107523 0.0025583697
0.0981547 0.0026651674
0.10228708 0.0027713136
0.10650467 0.0028766478
0.11080745 0.0029810221
0.11519545 0.0030843006
0.11966864 0.0031863596
0.12422704 0.0032870869
0.12887065 0.003386382
0.13359945 0.003484155
0.13841346 0.0035803269
0.14331268 0.0036748284
0.1482971 0.0037676
0.15336672 0.0038585911
0.15852155 0.0039477594
0.16376157 0.0040350709
0.16908681 0.0041204987
0.17449725 0.0042040229
0.17999289 0.0042856301
0.18557373 0.0043653127
0.19123978 0.0044430682
0.19699103 0.0045188996
0.20282749 0.0045928138
0.20874915 0.0046648222
0.21475601 0.0047349396
0.22084808 0.0048031842
0.22702535 0.0048695772
0.23328782 0.004934142
0.2396355 0.0049969048
0.24606838 0.0050578934
0.25258647 0.0051171375
0.25918976 0.0051746682
0.26587825 0.0052305179
0.27265195 0.0052847198
0.27951085 0.0053373081
0.28645495 0.0053883177
0.29348426 0.0054377839
0.30059877 0.0054857422
0.30779849 0.0055322284
0.3150834 0.0055772785
0.32245353 0.0056209282
0.32990885 0.0056632133
0.33744938 0.0057041693
0.34507512 0.0057438314
0.35278606 0.0057822343
0.3605822 0.0058194125
0.36846354 0.0058553999
0.37643009 0.0058902299
0.38448185 0.0059239353
0.3926188 0.0059565483
0.40084096 0.0059881005
0.40914833 0.006018623
0.41754089 0.0060481459
0.42601867 0.0060766989
0.43458164 0.0061043109
0.44322982 0.0061310102
0.4519632 0.0061568243
0.46078179 0.0061817799
0.46968558 0.0062059032
0.47867457 0.0062292196
0.48774877 0.0062517539
0.49690817 0.00627353
0.50615278 0.0062945713
0.51548258 0.0063149005
0.5248976 0.0063345396
0.53439781 0.00635351
0.54398323 0.0063718323
0.55365386 0.0063895267
0.56340968 0.0064066126
0.57325072 0.0064231089
0.58317695 0.0064390338
0.59318839 0.0064544051
0.60328503 0.00646924
0.61346688 0.0064835549
0.62373393 0.0064973659
0.63408618 0.0065106887
0.64452364 0.0065235381
0.6550463 0.0065359289
0.66565416 0.0065478749
0.67634723 0.0065593898
0.6871255 0.0065704868
0.69798898 0.0065811785
0.70893766 0.0065914773
0.71997154 0.006601395
0.73109063 0.006610943
0.74229492 0.0066201325
0.75358442 0.0066289742
0.76495911 0.0066374785
0.77641902 0.0066456552
0.78796412 0.0066535141
0.79959443 0.0066610646
0.81130995 0.0066683155
0.82311066 0.0066752757
0.83499658 0.0066819536
0.84696771 0.0066883572
0.85902404 0.0066944943
0.87116557 0.0067003727
0.8833923 0.0067059995
0.89570424 0.0067113819
0.90810139 0.0067165267
0.92058373 0.0067214405
0.93315128 0.0067261295
0.94580404 0.0067306001
0.958542 0.006734858
0.97136516 0.0067389091
0.98427352 0.0067427589
0.99726709 0.0067464126
1.0103459 0.0067498755
1.0235098 0.0067531526
1.036759 0.0067562487
1.0500934 0.0067591683
1.063513 0.0067619161
1.0770178 0.0067644963
1.0906078 0.0067669131
1.104283 0.0067691705
1.1180434 0.0067712726
1.131889 0.0067732229
1.1458198 0.0067750252
1.1598358 0.006776683
1.173937 0.0067781997
1.1881235 0.0067795786
1.2023951 0.0067808227
1.2167519 0.0067819353
1.2311939 0.0067829192
1.2457212 0.0067837772
1.2603336 0.0067845122
1.2750313 0.0067851268
1.2898141 0.0067856236
1.3046822 0.006786005
1.3196354 0.0067862735
1.3346739 0.0067864313
1.3497975 0.0067864808
1.3650064 0.0067864239
1.3803005 0.0067862629
1.3956797 0.0067859998
1.4111442 0.0067856364
1.4266939 0.0067851747
1.4423288 0.0067846165
1.4580489 0.0067839635
1.4738542 0.0067832175
1.4897447 0.0067823799
1.5057204 0.0067814525
1.5217813 0.0067804368
1.5379274 0.0067793341
1.5541587 0.006778146
1.5704752 0.0067768737
1.5868769 0.0067755187
1.6033638 0.0067740822
1.619936 0.0067725653
1.6365933 0.0067709694
1.6533358 0.0067692955
1.6701636 0.0067675448
1.6870765 0.0067657183
1.7040747 0.006763817
1.721158 0.0067618419
1.7383266 0.0067597941
1.7555803 0.0067576743
1.7729193 0.0067554836
1.7903434 0.0067532227
1.8078528 0.0067508925
1.8254474 0.0067484938
1.8431272 0.0067460273
1.8608921 0.0067434938
1.8787423 0.006740894
1.8966777 0.0067382286
1.9146983 0.0067354983
1.9328041 0.0067327036
1.9509951 0.0067298452
1.9692713 0.0067269237
1.9876327 0.0067239397
2.0060793 0.0067208937
2.0246111 0.0067177862
2.0432281 0.0067146177
2.0619303 0.0067113887
2.0807178 0.0067080997
2.0995904 0.0067047511
2.1185482 0.0067013434
2.1375913 0.006697877
2.1567195 0.0066943522
2.1759329 0.0066907695
2.1952316 0.0066871291
2.2146154 0.0066834316
2.2340845 0.0066796771
2.2536387 0.006675866
2.2732782 0.0066719986
2.2930029 0.0066680753
2.3128127 0.0066640963
2.3327078 0.0066600618
2.3526881 0.0066559721
2.3727536 0.0066518274
2.3929042 0.0066476281
2.4131401 0.0066433743
2.4334612 0.0066390662
2.4538675 0.006634704
2.474359 0.0066302879
2.4949357 0.0066258182
2.5155976 0.0066212948
2.5363447 0.0066167182
2.557177 0.0066120883
2.5780946 0.0066074053
2.5990973 0.0066026694
2.6201852 0.0065978807
2.6413583 0.0065930393
2.6626167 0.0065881453
2.6839602 0.0065831988
2.7053889 0.0065782
2.7269029 0.0065731489
2.748502 0.0065680457
2.7701864 0.0065628903
2.7919559 0.0065576829
2.8138107 0.0065524236
2.8357506 0.0065471123
2.8577758 0.0065417492
2.8798862 0.0065363343
2.9020817 0.0065308677
2.9243625 0.0065253493
2.9467285 0.0065197793
2.9691797 0.0065141577
2.9917161 0.0065084845
3.0143377 0.0065027597
3.0370445 0.0064969833
3.0598365 0.0064911554
3.0827137 0.006485276
3.1056761 0.006479345
3.1287237 0.0064733625
3.1518565 0.0064673286
3.1750745 0.0064612431
3.1983777 0.0064551061
3.2217662 0.0064489175
3.2452398 0.0064426774
3.2687986 0.0064363858
3.2924427 0.0064300426
3.3161719 0.0064236479
3.3399863 0.0064172015
3.363886 0.0064107035
3.3878708 0.0064041539
3.4119409 0.0063975526
3.4360961 0.0063908995
3.4603366 0.0063841948
3.4846623 0.0063774383
3.5090731 0.0063706299
3.5335692 0.0063637698
3.5581505 0.0063568578
3.582817 0.0063498938
3.6075687 0.0063428779
3.6324055 0.0063358101
3.6573276 0.0063286901
3.6823349 0.0063215182
3.7074274 0.006314294
3.7326051 0.0063070178
3.757868 0.0062996893
3.7832162 0.0062923086
3.8086495 0.0062848755
3.834168 0.0062773902
3.8597717 0.0062698524
3.8854606 0.0062622622
3.9112348 0.0062546195
3.9370941 0.0062469242
3.9630386 0.0062391764
3.9890684 0.0062313759
4.0151833 0.0062235227
4.0413835 0.0062156169
4.0676688 0.0062076582
4.0940394 0.0061996467
4.1204951 0.0061915823
4.1470361 0.006183465
4.1736623 0.0061752947
4.2003736 0.0061670714
4.2271702 0.006158795
4.254052 0.0061504655
4.281019 0.0061420828
4.3080711 0.006133647
4.3352085 0.0061251579
4.3624311 0.0061166154
4.3897389 0.0061080197
4.4171319 0.0060993706
4.4446101 0.006090668
4.4721735 0.006081912
4.4998221 0.0060731025
4.527556 0.0060642394
4.555375 0.0060553228
4.5832792 0.0060463525
4.6112686 0.0060373286
4.6393433 0.006028251
4.6675031 0.0060191197
4.6957481 0.0060099347
4.7240784 0.0060006958
4.7524938 0.0059914032
4.7809945 0.0059820567
4.8095803 0.0059726564
4.8382514 0.0059632022
4.8670076 0.0059536941
4.8958491 0.005944132
4.9247758 0.0059345161
4.9537876 0.0059248461
4.9828847 0.0059151222
5.012067 0.0059053443
5.0413345 0.0058955123
5.0706872 0.0058856264
5.1001251 0.0058756864
5.1296481 0.0058656924
5.1592564 0.0058556444
5.1889499 0.0058455423
5.2187286 0.0058353862
5.2485926 0.005825176
5.2785417 0.0058149118
5.308576 0.0058045936
5.3386955 0.0057942213
5.3689002 0.0057837951
5.3991902 0.0057733148
5.4295653 0.0057627806
5.4600256 0.0057521924
5.4905712 0.0057415502
5.5212019 0.0057308542
5.5519178 0.0057201042
5.582719 0.0057093003
5.6136053 0.0056984426
5.6445769 0.0056875311
5.6756337 0.0056765658
5.7067756 0.0056655467
5.7380028 0.0056544739
5.7693152 0.0056433475
5.8007127 0.0056321675
5.8321955 0.0056209339
5.8637635 0.0056096467
5.8954167 0.0055983061
5.9271551 0.0055869121
5.9589787 0.0055754647
5.9908875 0.005563964
6.0228815 0.0055524101
6.0549607 0.005540803
6.0871251 0.0055291428
6.1193747 0.0055174296
6.1517095 0.0055056635
6.1841295 0.0054938444
6.2166348 0.0054819726
6.2492252 0.0054700481
6.2819008 0.005458071
6.3146617 0.0054460413
6.3475077 0.0054339592
6.3804389 0.0054218248
6.4134554 0.0054096382
6.446557 0.0053973994
6.4797439 0.0053851086
6.513016 0.0053727658
6.5463732 0.0053603713
6.5798157 0.0053479251
6.6133433 0.0053354273
6.6469562 0.005322878
6.6806543 0.0053102775
6.7144376 0.0052976257
6.7483061 0.005284923
6.7822597 0.0052721692
6.8162986 0.0052593647
&
@target G0.S2
@type xy
4.2601867e-05 2.0286891e-06
0.00017040747 3.6015044e-05
0.0003834168 0.00021965225
0.00068162986 0.00093130937
0.0010650467 0.003583322
0.0015336672 0.015697605
0.0020874915 0.13440538
0.0027265195 1.8097152
0.0034507512 0.10743725
0.0042601867 0.044850247
0.0051548258 0.028155007
0.0061346688 0.020995117
0.0071997154 0.017156684
0.0083499658 0.014813075
0.00958542 0.013255242
0.010906078 0.012155987
0.012311939 0.011345256
0.013803005 0.010726638
0.015379274 0.010241715
0.017040747 0.0098531815
0.018787423 0.009536185
0.020619303 0.0092735766
0.022536387 0.0090531709
0.024538675 0.0088660901
0.026626167 0.0087057251
0.028798862 0.008567063
0.031056761 0.0084462387
0.033399863 0.0083402279
0.03582817 0.0082466341
0.03834168 0.0081635354
0.040940394 0.0080893749
0.043624311 0.0080228787
0.046393433 0.0079629962
0.049247758 0.0079088533
0.052187286 0.0078597181
0.055212019 0.0078149733
0.058321955 0.007774095
0.061517095 0.0077366363
0.064797439 0.0077022138
0.068162986 0.0076704967
0.071613738 0.0076411988
0.075149693 0.0076140708
0.078770851 0.0075888952
0.082477214 0.0075654811
0.08626878 0.0075436605
0.09014555 0.0075232852
0.094107523 0.0075042236
0.0981547 0.0074863591
0.10228708 0.0074695876
0.10650467 0.0074538159
0.11080745 0.0074389609
0.11519545 0.0074249476
0.11966864 0.0074117086
0.12422704 0.007399183
0.12887065 0.0073873159
0.13359945 0.0073760572
0.13841346 0.0073653618
0.14331268 0.0073551883
0.1482971 0.0073454991
0.15336672 0.0073362601
0.15852155 0.0073274396
0.16376157 0.0073190089
0.16908681 0.0073109417
0.17449725 0.0073032136
0.17999289 0.0072958023
0.18557373 0.0072886872
0.19123978 0.0072818492
0.19699103 0.0072752707
0.20282749 0.0072689354
0.20874915 0.0072628284
0.21475601 0.0072569355
0.22084808 0.0072512437
0.22702535 0.0072457409
0.23328782 0.007240416
0.2396355 0.0072352582
0.24606838 0.007230258
0.25258647 0.007225406
0.25918976 0.0072206938
0.26587825 0.0072161132
0.27265195 0.0072116569
0.27951085 0.0072073177
0.28645495 0.0072030891
0.29348426 0.0071989648
0.30059877 0.007194939
0.30779849 0.0071910062
0.3150834 0.0071871611
0.32245353 0.0071833991
0.32990885 0.0071797153
0.33744938 0.0071761055
0.34507512 0.0071725655
0.35278606 0.0071690916
0.3605822 0.0071656799
0.36846354 0.007162327
0.37643009 0.0071590296
0.38448185 0.0071557846
0.3926188 0.007152589
0.40084096 0.0071494399
0.40914833 0.0071463347
0.41754089 0.0071432709
0.42601867 0.0071402459
0.43458164 0.0071372575
0.44322982 0.0071343035
0.4519632 0.0071313817
0.46078179 0.0071284902
0.46968558 0.007125627
0.47867457 0.0071227903
0.48774877 0.0071199784
0.49690817 0.0071171895
0.50615278 0.007114422
0.51548258 0.0071116745
0.5248976 0.0071089454
0.53439781 0.0071062334
0.54398323 0.007103537
0.55365386 0.0071008549
0.56340968 0.007098186
0.57325072 0.0070955289
0.58317695 0.0070928826
0.59318839 0.0070902459
0.60328503 0.0070876177
0.61346688 0.0070849971
0.62373393 0.0070823829
0.63408618 0.0070797743
0.64452364 0.0070771703
0.6550463 0.00707457
0.66565416 0.0070719726
0.67634723 0.0070693771
0.6871255 0.0070667828
0.69798898 0.0070641889
0.70893766 0.0070615946
0.71997154 0.0070589993
0.73109063 0.007056402
0.74229492 0.0070538023
0.75358442 0.0070511993
0.76495911 0.0070485925
0.77641902 0.0070459812
0.78796412 0.0070433647
0.79959443 0.0070407425
0.81130995 0.007038114
0.82311066 0.0070354786
0.83499658 0.0070328358
0.84696771 0.0070301849
0.85902404 0.0070275255
0.87116557 0.0070248571
0.8833923 0.0070221791
0.89570424 0.0070194911
0.90810139 0.0070167925
0.92058373 0.0070140829
0.93315128 0.0070113618
0.94580404 0.0070086288
0.958542 0.0070058834
0.97136516 0.0070031252
0.98427352 0.0070003538
0.99726709 0.0069975687
1.0103459 0.0069947695
1.0235098 0.0069919559
1.036759 0.0069891274
1.0500934 0.0069862836
1.063513 0.0069834242
1.0770178 0.0069805488
1.0906078 0.006977657
1.104283 0.0069747484
1.1180434 0.0069718227
1.131889 0.0069688796
1.1458198 0.0069659186
1.1598358 0.0069629395
1.173937 0.0069599418
1.1881235 0.0069569254
1.2023951 0.0069538897
1.2167519 0.0069508346
1.2311939 0.0069477597
1.2457212 0.0069446647
1.2603336 0.0069415492
1.2750313 0.0069384129
1.2898141 0.0069352556
1.3046822 0.0069320769
1.3196354 0.0069288766
1.3346739 0.0069256543
1.3497975 0.0069224098
1.3650064 0.0069191427
1.3803005 0.0069158527
1.3956797 0.0069125397
1.4111442 0.0069092032
1.4266939 0.0069058431
1.4423288 0.006902459
1.4580489 0.0068990507
1.4738542 0.0068956178
1.4897447 0.0068921602
1.5057204 0.0068886775
1.5217813 0.0068851695
1.5379274 0.0068816359
1.5541587 0.0068780764
1.5704752 0.0068744909
1.5868769 0.006870879
1.6033638 0.0068672404
1.619936 0.006863575
1.6365933 0.0068598824
1.6533358 0.0068561624
1.6701636 0.0068524148
1.6870765 0.0068486392
1.7040747 0.0068448356
1.721158 0.0068410035
1.7383266 0.0068371428
1.7555803 0.0068332532
1.7729193 0.0068293345
1.7903434 0.0068253865
1.8078528 0.0068214088
1.8254474 0.0068174012
1.8431272 0.0068133636
1.8608921 0.0068092956
1.8787423 0.0068051971
1.8966777 0.0068010678
1.9146983 0.0067969074
1.9328041 0.0067927158
1.9509951 0.0067884927
1.9692713 0.0067842378
1.9876327 0.006779951
2.0060793 0.006775632
2.0246111 0.0067712806
2.0432281 0.0067668965
2.0619303 0.0067624796
2.0807178 0.0067580296
2.0995904 0.0067535462
2.1185482 0.0067490293
2.1375913 0.0067444786
2.1567195 0.006739894
2.1759329 0.0067352751
2.1952316 0.0067306218
2.2146154 0.0067259339
2.2340845 0.0067212111
2.2536387 0.0067164532
2.2732782 0.0067116599
2.2930029 0.0067068312
2.3128127 0.0067019668
2.3327078 0.0066970664
2.3526881 0.0066921298
2.3727536 0.0066871569
2.3929042 0.0066821473
2.4131401 0.006677101
2.4334612 0.0066720177
2.4538675 0.0066668971
2.474359 0.0066617392
2.4949357 0.0066565436
2.5155976 0.0066513101
2.5363447 0.0066460387
2.557177 0.0066407289
2.5780946 0.0066353808
2.5990973 0.0066299939
2.6201852 0.0066245682
2.6413583 0.0066191035
2.6626167 0.0066135995
2.6839602 0.006608056
2.7053889 0.0066024729
2.7269029 0.0065968499
2.748502 0.0065911869
2.7701864 0.0065854836
2.7919559 0.0065797399
2.8138107 0.0065739556
2.8357506 0.0065681304
2.8577758 0.0065622642
2.8798862 0.0065563568
2.9020817 0.006550408
2.9243625 0.0065444176
2.9467285 0.0065383854
2.9691797 0.0065323112
2.9917161 0.0065261949
3.0143377 0.0065200363
3.0370445 0.0065138351
3.0598365 0.0065075913
3.0827137 0.0065013045
3.1056761 0.0064949747
3.1287237 0.0064886016
3.1518565 0.0064821851
3.1750745 0.0064757251
3.1983777 0.0064692212
3.2217662 0.0064626734
3.2452398 0.0064560814
3.2687986 0.0064494452
3.2924427 0.0064427645
3.3161719 0.0064360391
3.3399863 0.006429269
3.363886 0.0064224539
3.3878708 0.0064155936
3.4119409 0.006408688
3.4360961 0.006401737
3.4603366 0.0063947403
3.4846623 0.0063876978
3.5090731 0.0063806094
3.5335692 0.0063734748
3.5581505 0.006366294
3.582817 0.0063590668
3.6075687 0.006351793
3.6324055 0.0063444725
3.6573276 0.0063371051
3.6823349 0.0063296906
3.7074274 0.006322229
3.7326051 0.0063147201
3.757868 0.0063071637
3.7832162 0.0062995597
3.8086495 0.0062919079
3.834168 0.0062842082
3.8597717 0.0062764605
3.8854606 0.0062686647
3.9112348 0.0062608205
3.9370941 0.0062529279
3.9630386 0.0062449867
3.9890684 0.0062369969
4.0151833 0.0062289582
4.0413835 0.0062208705
4.0676688 0.0062127338
4.0940394 0.0062045479
4.1204951 0.0061963126
4.1470361 0.006188028
4.1736623 0.0061796937
4.2003736 0.0061713098
4.2271702 0.0061628761
4.254052 0.0061543925
4.281019 0.0061458589
4.3080711 0.0061372752
4.3352085 0.0061286413
4.3624311 0.006119957
4.3897389 0.0061112224
4.4171319 0.0061024372
4.4446101 0.0060936013
4.4721735 0.0060847148
4.4998221 0.0060757774
4.527556 0.0060667892
4.555375 0.00605775
4.5832792 0.0060486597
4.6112686 0.0060395182
4.6393433 0.0060303255
4.6675031 0.0060210815
4.6957481 0.006011786
4.7240784 0.0060024391
4.7524938 0.0059930407
4.7809945 0.0059835906
4.8095803 0.0059740889
4.8382514 0.0059645354
4.8670076 0.0059549301
4.8958491 0.0059452729
4.9247758 0.0059355638
4.9537876 0.0059258027
4.9828847 0.0059159896
5.012067 0.0059061243
5.0413345 0.005896207
5.0706872 0.0058862374
5.1001251 0.0058762156
5.1296481 0.0058661416
5.1592564 0.0058560152
5.1889499 0.0058458365
5.2187286 0.0058356054
5.2485926 0.0058253219
5.2785417 0.005814986
5.308576 0.0058045977
5.3386955 0.0057941568
5.3689002 0.0057836635
5.3991902 0.0057731176
5.4295653 0.0057625192
5.4600256 0.0057518683
5.4905712 0.0057411649
5.5212019 0.0057304089
5.5519178 0.0057196003
5.582719 0.0057087392
5.6136053 0.0056978256
5.6445769 0.0056868594
5.6756337 0.0056758407
5.7067756 0.0056647695
5.7380028 0.0056536458
5.7693152 0.0056424696
5.8007127 0.005631241
5.8321955 0.0056199599
5.8637635 0.0056086265
5.8954167 0.0055972406
5.9271551 0.0055858025
5.9589787 0.005574312
5.9908875 0.0055627694
6.0228815 0.0055511745
6.0549607 0.0055395274
6.0871251 0.0055278282
6.1193747 0.005516077
6.1517095 0.0055042738
6.1841295 0.0054924187
6.2166348 0.0054805117
6.2492252 0.0054685528
6.2819008 0.0054565423
6.3146617 0.0054444801
6.3475077 0.0054323663
6.3804389 0.0054202011
6.4134554 0.0054079844
6.446557 0.0053957164
6.4797439 0.0053833972
6.513016 0.0053710268
6.5463732 0.0053586054
6.5798157 0.0053461331
6.6133433 0.0053336099
6.6469562 0.005321036
6.6806543 0.0053084115
6.7144376 0.0052957366
6.7483061 0.0052830112
6.7822597 0.0052702356
6.8162986 0.0052574099
&
@target G1.S1
@type xy
4.2601863e-07 1.9625324e-10
1.7040745e-06 3.1431829e-09
3.8341677e-06 1.5938834e-08
6.8162981e-06 5.0492064e-08
1.0650466e-05 1.2364187e-07
1.5336671e-05 2.5732681e-07
2.0874913e-05 4.7880684e-07
2.7265193e-05 8.2094088e-07
3.4507509e-05 1.3225239e-06
4.2601863e-05 2.0286888e-06
5.1548255e-05 2.9913783e-06
6.1346683e-05 4.269895e-06
7.1997149e-05 5.9315367e-06
8.3499652e-05 8.0523284e-06
9.5854192e-05 1.0717861e-05
0.00010906077 1.402425e-05
0.00012311939 1.8079235e-05
0.00013803004 2.3003428e-05
0.00015379273 2.8931746e-05
0.00017040745 3.6015038e-05
0.00018787422 4.4421954e-05
0.00020619302 5.4341071e-05
0.00022536386 6.5983336e-05
0.00024538673 7.958486e-05
0.00026626165 9.541013e-05
0.0002879886 0.0001137557
0.00031056758 0.00013495445
0.00033399861 0.00015938049
0.00035828167 0.00018745489
0.00038341677 0.00021965221
0.00040940391 0.00025650825
0.00043624308 0.00029862899
0.00046393429 0.00034670105
0.00049247754 0.000401504
0.00052187283 0.00046392485
0.00055212015 0.00053497516
0.00058321951 0.00061581123
0.00061517091 0.00070775831
0.00064797434 0.00081233927
0.00068162981 0.00093130918
0.00071613732 0.0010666968
0.00075149687 0.001220855
0.00078770845 0.0013965215
0.00082477207 0.0015968937
0.00086268773 0.0018257204
0.00090145543 0.0020874147
0.00094107516 0.0023871945
0.00098154693 0.0027312583
0.0010228707 0.0031270064
0.0010650466 0.0035833211
0.0011080745 0.0041109253
0.0011519544 0.0047228433
0.0011966863 0.0054350013
0.0012422703 0.006267014
0.0012887064 0.0072432283
0.0013359944 0.0083941221
0.0013841345 0.0097582025
0.0014331267 0.011384616
0.0014829709 0.013336792
0.0015336671 0.015697599
0.0015852153 0.018576795
0.0016376156 0.022121972
0.001690868 0.026535015
0.0017449723 0.032097439
0.0017999287 0.039210502
0.0018557372 0.048460731
0.0019123976 0.060730873
0.0019699102 0.077395863
0.0020282747 0.10068648
0.0020874913 0.13440527
0.0021475599 0.1854412
0.0022084806 0.26727368
0.0022702533 0.40905826
0.002332878 0.6829967
0.0023963548 1.3053605
0.0024606836 3.1242151
0.0025258645 10.107371
0.0025918974 12.78454
0.0026587823 4.237332
0.0027265193 1.809719
0.0027951083 0.98986977
0.0028645493 0.62772446
0.0029348424 0.43731055
0.0030059875 0.32485705
0.0030779846 0.25277084
0.0031508338 0.20367173
0.003224535 0.16863493
0.0032990883 0.14269462
0.0033744936 0.12290743
0.0034507509 0.1074373
0.0035278603 0.095089656
0.0036058217 0.085059357
0.0036846352 0.076787187
0.0037643006 0.069874573
0.0038448182 0.064030986
0.0039261877 0.059040428
0.0040084093 0.054739486
0.004091483 0.051002596
0.0041754086 0.047731919
0.0042601863 0.044850257
0.0043458161 0.042296002
0.0044322979 0.040019472
0.0045196317 0.037980225
0.0046078175 0.03614505
0.0046968554 0.034486458
0.0047867454 0.032981524
0.0048774873 0.031611
0.0049690813 0.030358622
0.0050615274 0.029210565
0.0051548255 0.028155011
0.0052489756 0.027181808
0.0053439777 0.026282191
0.0054398319 0.025448558
0.0055365382 0.024674285
0.0056340964 0.023953582
0.0057325067 0.023281365
0.0058317691 0.022653153
0.0059318835 0.022064986
0.0060328499 0.02151335
0.0061346683 0.020995119
0.0062373388 0.020507504
0.0063408613 0.020048007
0.0064452359 0.01961439
0.0065504625 0.019204636
0.0066565411 0.01881693
0.0067634718 0.018449628
0.0068712545 0.018101244
0.0069798893 0.017770426
0.0070893761 0.017455947
0.0071997149 0.017156686
0.0073109058 0.016871621
0.0074229487 0.016599816
0.0075358436 0.016340415
0.0076495906 0.016092631
0.0077641896 0.015855739
0.0078796406 0.015629075
0.0079959437 0.015412023
0.0081130989 0.015204016
0.008231106 0.015004529
0.0083499652 0.014813076
0.0084696764 0.014629207
0.0085902397 0.014452503
0.008711655 0.014282574
0.0088339224 0.014119059
0.0089570418 0.01396162
0.0090810132 0.013809942
0.0092058366 0.013663732
0.0093315121 0.013522714
0.0094580397 0.013386631
0.0095854192 0.013255243
0.0097136509 0.013128323
0.0098427345 0.01300566
0.0099726702 0.012887054
0.010103458 0.012772318
0.010235098 0.012661276
0.010367589 0.012553762
0.010500933 0.012449619
0.010635129 0.012348701
0.010770177 0.012250867
0.010906077 0.012155987
0.011042829 0.012063936
0.011180433 0.011974596
0.011318889 0.011887856
0.011458197 0.01180361
0.011598357 0.011721758
0.011739369 0.011642206
0.011881234 0.011564863
0.01202395 0.011489644
0.012167518 0.011416468
0.012311939 0.011345257
0.012457211 0.011275937
0.012603335 0.011208439
0.012750312 0.011142695
0.01289814 0.011078643
0.013046821 0.011016222
0.013196353 0.010955373
0.013346738 0.010896042
0.013497974 0.010838176
0.013650063 0.010781724
0.013803004 0.010726639
0.013956796 0.010672874
0.014111441 0.010620385
0.014266938 0.010569131
0.014423287 0.01051907
0.014580488 0.010470164
0.014738541 0.010422376
0.014897446 0.010375671
0.015057203 0.010330014
0.015217812 0.010285372
0.015379273 0.010241715
0.015541586 0.010199012
0.015704751 0.010157234
0.015868768 0.010116353
0.016033637 0.010076342
0.016199359 0.010037176
0.016365932 0.0099988303
0.016533357 0.0099612803
0.016701635 0.0099245036
0.016870764 0.0098884778
0.017040745 0.0098531817
0.017211579 0.0098185949
0.017383264 0.0097846975
0.017555802 0.0097514705
0.017729191 0.0097188955
0.017903433 0.0096869547
0.018078527 0.0096556311
0.018254472 0.009624908
0.01843127 0.0095947695
0.01860892 0.0095652002
0.018787422 0.0095361852
0.018966776 0.0095077101
0.019146981 0.009479761
0.019328039 0.0094523244
0.019509949 0.0094253873
0.019692711 0.0093989371
0.019876325 0.0093729617
0.020060791 0.0093474492
0.02024611 0.0093223882
0.02043228 0.0092977676
0.020619302 0.0092735768
0.020807176 0.0092498053
0.020995902 0.0092264432
0.021185481 0.0092034806
0.021375911 0.0091809081
0.021567193 0.0091587166
0.021759328 0.0091368971
0.021952314 0.0091154411
0.022146153 0.0090943401
0.022340843 0.0090735861
0.022536386 0.0090531711
0.02273278 0.0090330876
0.022930027 0.009013328
0.023128126 0.0089938852
0.023327076 0.0089747522
0.023526879 0.0089559221
0.023727534 0.0089373883
0.023929041 0.0089191444
0.024131399 0.0089011841
0.02433461 0.0088835014
0.024538673 0.0088660903
0.024743588 0.008848945
0.024949355 0.00883206
0.025155974 0.0088154298
0.025363445 0.0087990492
0.025571768 0.0087829129
0.025780944 0.0087670159
0.025990971 0.0087513533
0.02620185 0.0087359205
0.026413581 0.0087207126
0.026626165 0.0087057252
0.0268396 0.008690954
0.027053887 0.0086763945
0.027269027 0.0086620427
0.027485018 0.0086478944
0.027701862 0.0086339457
0.027919557 0.0086201926
0.028138105 0.0086066315
0.028357504 0.0085932586
0.028577756 0.0085800703
0.02879886 0.0085670632
0.029020815 0.0085542337
0.029243623 0.0085415786
0.029467283 0.0085290946
0.029691795 0.0085167784
0.029917159 0.0085046271
0.030143374 0.0084926376
0.030370442 0.0084808068
0.030598362 0.008469132
0.030827134 0.0084576102
0.031056758 0.0084462388
0.031287234 0.008435015
0.031518563 0.0084239362
0.031750743 0.0084129998
0.031983775 0.0084022033
0.032217659 0.0083915442
0.032452395 0.0083810201
0.032687984 0.0083706288
0.032924424 0.0083603678
0.033161716 0.008350235
0.033399861 0.008340228
0.033638857 0.0083303449
0.033878706 0.0083205835
0.034119406 0.0083109416
0.034360959 0.0083014174
0.034603363 0.0082920088
0.03484662 0.0082827139
0.035090729 0.0082735308
0.03533569 0.0082644577
0.035581502 0.0082554928
0.035828167 0.0082466342
0.036075684 0.0082378803
0.036324053 0.0082292293
0.036573274 0.0082206797
0.036823347 0.0082122297
0.037074272 0.0082038778
0.037326049 0.0081956223
0.037578678 0.0081874619
0.037832159 0.0081793949
0.038086492 0.0081714199
0.038341677 0.0081635355
0.038597714 0.0081557403
0.038854603 0.0081480328
0.039112345 0.0081404117
0.039370938 0.0081328757
0.039630383 0.0081254234
0.039890681 0.0081180537
0.04015183 0.0081107652
0.040413832 0.0081035567
0.040676685 0.008096427
0.040940391 0.008089375
0.041204948 0.0080823994
0.041470358 0.0080754991
0.041736619 0.008068673
0.042003733 0.0080619201
0.042271699 0.0080552391
0.042540517 0.0080486292
0.042810186 0.0080420892
0.043080708 0.0080356181
0.043352082 0.008029215
0.043624308 0.0080228788
0.043897386 0.0080166086
0.044171316 0.0080104035
0.044446098 0.0080042625
0.044721732 0.0079981847
0.044998218 0.0079921692
0.045275556 0.0079862151
0.045553746 0.0079803216
0.045832789 0.0079744879
0.046112683 0.007968713
0.046393429 0.0079629963
0.046675027 0.0079573368
0.046957478 0.0079517338
0.04724078 0.0079461865
0.047524935 0.0079406942
0.047809941 0.0079352561
0.0480958 0.0079298715
0.04838251 0.0079245396
0.048670073 0.0079192597
0.048958487 0.0079140312
0.049247754 0.0079088534
0.049537873 0.0079037255
0.049828843 0.007898647
0.050120666 0.0078936171
0.050413341 0.0078886353
0.050706868 0.0078837008
0.051001247 0.0078788132
0.051296478 0.0078739717
0.051592561 0.0078691757
0.051889496 0.0078644247
0.052187283 0.0078597182
0.052485922 0.0078550554
0.052785413 0.007850436
0.053085756 0.0078458592
0.053386951 0.0078413246
0.053688998 0.0078368317
0.053991898 0.0078323798
0.054295649 0.0078279686
0.054600252 0.0078235974
0.054905707 0.0078192658
0.055212015 0.0078149733
0.055519174 0.0078107194
0.055827186 0.0078065037
0.056136049 0.0078023255
0.056445765 0.0077981846
0.056756332 0.0077940804
0.057067752 0.0077900125
0.057380024 0.0077859805
0.057693147 0.0077819838
0.058007123 0.0077780221
0.058321951 0.007774095
0.058637631 0.0077702021
0.058954163 0.0077663428
0.059271546 0.0077625169
0.059589782 0.007758724
0.05990887 0.0077549636
0.06022881 0.0077512353
0.060549602 0.0077475388
0.060871246 0.0077438737
0.061193743 0.0077402397
0.061517091 0.0077366364
0.061841291 0.0077330633
0.062166343 0.0077295202
0.062492247 0.0077260068
0.062819004 0.0077225226
0.063146612 0.0077190674
0.063475072 0.0077156407
0.063804385 0.0077122424
0.064134549 0.007708872
0.064465566 0.0077055292
0.064797434 0.0077022138
0.065130155 0.0076989254
0.065463727 0.0076956637
0.065798152 0.0076924284
0.066133429 0.0076892193
0.066469557 0.0076860359
0.066806538 0.0076828781
0.067144371 0.0076797456
0.067483056 0.007676638
0.067822592 0.0076735552
0.068162981 0.0076704968
&


==> rev_plot <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 20 to "Dingbats-Regular", "Dingbats-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 25 to "NimbusMonoL-Bold", "NimbusMonoL-Bold"
@map font 26 to "NimbusMonoL-BoldOblique", "NimbusMonoL-BoldOblique"
@map font 27 to "NimbusMonoL-Regular", "NimbusMonoL-Regular"
@map font 28 to "NimbusMonoL-RegularOblique", "NimbusMonoL-RegularOblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 37 to "NimbusRomanNo9L-Medium", "NimbusRomanNo9L-Medium"
@map font 38 to "NimbusRomanNo9L-MediumItalic", "NimbusRomanNo9L-MediumItalic"
@map font 39 to "NimbusRomanNo9L-Regular", "NimbusRomanNo9L-Regular"
@map font 40 to "NimbusRomanNo9L-RegularItalic", "NimbusRomanNo9L-RegularItalic"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 45 to "NimbusSansL-Bold", "NimbusSansL-Bold"
@map font 46 to "NimbusSansL-BoldCondensed", "NimbusSansL-BoldCondensed"
@map font 47 to "NimbusSansL-BoldCondensedItalic", "NimbusSansL-BoldCondensedItalic"
@map font 48 to "NimbusSansL-BoldItalic", "NimbusSansL-BoldItalic"
@map font 49 to "NimbusSansL-Regular", "NimbusSansL-Regular"
@map font 50 to "NimbusSansL-RegularCondensed", "NimbusSansL-RegularCondensed"
@map font 51 to "NimbusSansL-RegularCondensedItalic", "NimbusSansL-RegularCondensedItalic"
@map font 52 to "NimbusSansL-RegularItalic", "NimbusSansL-RegularItalic"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 61 to "StandardSymbolsL-Regular", "StandardSymbolsL-Regular"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 72 to "URWBookmanL-DemiBold", "URWBookmanL-DemiBold"
@map font 73 to "URWBookmanL-DemiBoldItalic", "URWBookmanL-DemiBoldItalic"
@map font 74 to "URWBookmanL-Light", "URWBookmanL-Light"
@map font 75 to "URWBookmanL-LightItalic", "URWBookmanL-LightItalic"
@map font 76 to "URWChanceryL-MediumItalic", "URWChanceryL-MediumItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 81 to "URWGothicL-Book", "URWGothicL-Book"
@map font 82 to "URWGothicL-BookOblique", "URWGothicL-BookOblique"
@map font 83 to "URWGothicL-Demi", "URWGothicL-Demi"
@map font 84 to "URWGothicL-DemiOblique", "URWGothicL-DemiOblique"
@map font 85 to "URWPalladioL-Bold", "URWPalladioL-Bold"
@map font 86 to "URWPalladioL-BoldItalic", "URWPalladioL-BoldItalic"
@map font 87 to "URWPalladioL-Italic", "URWPalladioL-Italic"
@map font 88 to "URWPalladioL-Roman", "URWPalladioL-Roman"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Sep 13 12:32:57 2021"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, 100, 13, 180
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.244118, 0.950000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "T\slab\N [MeV]"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.500000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 2
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.500000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "\xd\0(\S3\NP\s0\N) [deg]"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.500000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 10
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.500000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.85, 0.8
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.000000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 2
@    s0 symbol pattern 1
@    s0 symbol fill color 2
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 2
@    s0 line linewidth 3.5
@    s0 line color 2
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 2
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/chiehjen/jerry/test_per/676_lo"
@    s0 legend  "LO"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 0
@    s1 symbol size 1.000000
@    s1 symbol color 1
@    s1 symbol pattern 1
@    s1 symbol fill color 1
@    s1 symbol fill pattern 0
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 1
@    s1 line linestyle 1
@    s1 line linewidth 1.5
@    s1 line color 1
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 1
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "919_nlo_nonper"
@    s1 legend  "NLO non-per"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 1
@    s2 symbol size 0.500000
@    s2 symbol color 4
@    s2 symbol pattern 1
@    s2 symbol fill color 4
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 5
@    s2 line type 0
@    s2 line linestyle 3
@    s2 line linewidth 1.5
@    s2 line color 4
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 4
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/chiehjen/jerry/test_per/919_nlo"
@    s2 legend  "NLO per"
@target G0.S0
@type xy
8.5203735e-05 179.99996
0.00034081494 179.99967
0.00076683362 179.99888
0.0013632598 179.99735
0.0021300934 179.99483
0.0030673345 179.99109
0.004174983 179.98591
0.0054530391 179.97904
0.0069015026 179.97029
0.0085203735 179.95945
0.010309652 179.94632
0.012269338 179.93071
0.014399431 179.91246
0.016699932 179.89141
0.01917084 179.8674
0.021812156 179.84031
0.02462388 179.81001
0.02760601 179.77638
0.030758548 179.73935
0.034081494 179.69882
0.037574847 179.65472
0.041238608 179.607
0.045072776 179.55561
0.049077352 179.50052
0.053252335 179.4417
0.057597725 179.37915
0.062113523 179.31286
0.066799728 179.24285
0.071656341 179.16912
0.076683362 179.09171
0.08188079 179.01065
0.087248625 178.92599
0.092786868 178.83776
0.098495518 178.74602
0.10437458 178.65084
0.11042404 178.55228
0.11664391 178.4504
0.12303419 178.34528
0.12959488 178.23699
0.13632598 178.12561
0.14322748 178.01123
0.15029939 177.89391
0.15754171 177.77375
0.16495443 177.65083
0.17253756 177.52523
0.1802911 177.39704
0.18821505 177.26634
0.19630941 177.13322
0.20457417 176.99775
0.21300934 176.86003
0.22161492 176.72014
0.2303909 176.57815
0.23933729 176.43415
0.24845409 176.28821
0.2577413 176.14041
0.26719891 175.99083
0.27682694 175.83953
0.28662537 175.68659
0.2965942 175.53208
0.30673345 175.37606
0.3170431 175.21861
0.32752316 175.05977
0.33817363 174.89962
0.3489945 174.73822
0.35998578 174.57561
0.37114747 174.41187
0.38247957 174.24703
0.39398207 174.08115
0.40565498 173.91429
0.4174983 173.74649
0.42951203 173.57779
0.44169616 173.40824
0.45405071 173.23788
0.46657565 173.06676
0.47927101 172.8949
0.49213678 172.72236
0.50517295 172.54916
0.51837953 172.37533
0.53175651 172.20093
0.54530391 172.02596
0.55902171 171.85047
0.57290992 171.67447
0.58696853 171.49801
0.60119756 171.32111
0.61559699 171.14378
0.63016683 170.96606
0.64490707 170.78796
0.65981773 170.60951
0.67489879 170.43073
0.69015026 170.25164
0.70557213 170.07226
0.72116442 169.8926
0.73692711 169.71268
0.75286021 169.53252
0.76896371 169.35213
0.78523762 169.17153
0.80168195 168.99073
0.81829667 168.80974
0.83508181 168.62857
0.85203735 168.44725
0.8691633 168.26577
0.88645966 168.08415
0.90392643 167.90239
0.9215636 167.72052
0.93937118 167.53853
0.95734917 167.35643
0.97549757 167.17424
0.99381637 166.99195
1.0123056 166.80958
1.0309652 166.62714
1.0497952 166.44462
1.0687957 166.26203
1.0879665 166.07939
1.1073077 165.89669
1.1268194 165.71394
1.1465015 165.53114
1.1663539 165.3483
1.1863768 165.16542
1.2065701 164.9825
1.2269338 164.79955
1.2474679 164.61658
1.2681724 164.43357
1.2890473 164.25055
1.3100926 164.0675
1.3313084 163.88443
1.3526945 163.70134
1.374251 163.51824
1.395978 163.33512
1.4178754 163.15199
1.4399431 162.96885
1.4621813 162.7857
1.4845899 162.60254
1.5071689 162.41937
1.5299183 162.23619
1.5528381 162.053
1.5759283 161.86981
1.5991889 161.68661
1.6226199 161.5034
1.6462214 161.32019
1.6699932 161.13697
1.6939355 160.95375
1.7180481 160.77051
1.7423312 160.58728
1.7667847 160.40403
1.7914085 160.22078
1.8162028 160.03752
1.8411675 159.85425
1.8663026 159.67097
1.8916081 159.48769
1.917084 159.30439
1.9427304 159.12109
1.9685471 158.93777
1.9945342 158.75444
2.0206918 158.5711
2.0470197 158.38775
2.0735181 158.20438
2.1001869 158.02099
2.127026 157.83759
2.1540356 157.65417
2.1812156 157.47073
2.208566 157.28728
2.2360868 157.1038
2.263778 156.9203
2.2916397 156.73678
2.3196717 156.55323
2.3478741 156.36966
2.376247 156.18607
2.4047902 156.00244
2.4335039 155.81879
2.462388 155.63511
2.4914424 155.45139
2.5206673 155.26765
2.5500626 155.08387
2.5796283 154.90006
2.6093644 154.71621
2.6392709 154.53232
2.6693478 154.34839
2.6995951 154.16443
2.7300129 153.98042
2.760601 153.79637
2.7913596 153.61228
2.8222885 153.42814
2.8533879 153.24395
2.8846577 153.05972
2.9160978 152.87544
2.9477084 152.69111
2.9794894 152.50672
3.0114408 152.32229
3.0435626 152.1378
3.0758548 151.95325
3.1083175 151.76865
3.1409505 151.58399
3.1737539 151.39926
3.2067278 151.21448
3.239872 151.02964
3.2731867 150.84473
3.3066718 150.65976
3.3403272 150.47472
3.3741531 150.28962
3.4081494 150.10444
3.4423161 149.9192
3.4766532 149.73389
3.5111607 149.5485
3.5458386 149.36304
3.580687 149.1775
3.6157057 148.99189
3.6508949 148.8062
3.6862544 148.62044
3.7217844 148.43459
3.7574847 148.24866
3.7933555 148.06265
3.8293967 147.87656
3.8656083 147.69038
3.9019903 147.50412
3.9385427 147.31777
3.9752655 147.13133
4.0121587 146.9448
4.0492223 146.75818
4.0864563 146.57147
4.1238608 146.38466
4.1614356 146.19776
4.1991809 146.01077
4.2370966 145.82368
4.2751826 145.63649
4.3134391 145.44921
4.351866 145.26182
4.3904633 145.07434
4.429231 144.88675
4.4681691 144.69906
4.5072776 144.51126
4.5465565 144.32336
4.5860058 144.13536
4.6256256 143.94724
4.6654157 143.75902
4.7053763 143.57069
4.7455072 143.38225
4.7858086 143.1937
4.8262804 143.00503
4.8669226 142.81625
4.9077352 142.62736
4.9487182 142.43835
4.9898716 142.24922
5.0311954 142.05998
5.0726896 141.87062
5.1143542 141.68114
5.1561892 141.49154
5.1981947 141.30182
5.2403705 141.11197
5.2827168 140.922
5.3252335 140.73191
5.3679205 140.5417
5.410778 140.35135
5.4538059 140.16088
5.4970042 139.97029
5.5403729 139.77956
5.583912 139.58871
5.6276215 139.39772
5.6715014 139.2066
5.7155518 139.01535
5.7597725 138.82397
5.8041637 138.63246
5.8487252 138.44081
5.8934572 138.24902
5.9383595 138.0571
5.9834323 137.86504
6.0286755 137.67284
6.0740891 137.48051
6.1196731 137.28803
6.1654275 137.09542
6.2113523 136.90266
6.2574475 136.70976
6.3037132 136.51672
6.3501492 136.32354
6.3967556 136.13021
6.4435325 135.93673
6.4904797 135.74312
6.5375974 135.54935
6.5848855 135.35544
6.632344 135.16138
6.6799728 134.96717
6.7277721 134.77281
6.7757418 134.57831
6.823882 134.38365
6.8721925 134.18884
6.9206734 133.99388
6.9693247 133.79877
7.0181465 133.6035
7.0671386 133.40808
7.1163012 133.21251
7.1656341 133.01678
7.2151375 132.82089
7.2648113 132.62485
7.3146555 132.42865
7.3646701 132.2323
7.4148551 132.03578
7.4652105 131.83911
7.5157363 131.64228
7.5664325 131.44529
7.6172991 131.24813
7.6683362 131.05082
7.7195436 130.85335
7.7709215 130.65571
7.8224697 130.45791
7.8741884 130.25995
7.9260775 130.06182
7.978137 129.86353
8.0303668 129.66507
8.0827671 129.46645
8.1353379 129.26767
8.188079 129.06872
8.2409905 128.8696
8.2940724 128.67031
8.3473247 128.47086
8.4007475 128.27123
8.4543406 128.07144
8.5081042 127.87148
8.5620382 127.67135
8.6161425 127.47106
8.6704173 127.27059
8.7248625 127.06995
8.7794781 126.86913
8.8342641 126.66815
8.8892205 126.467
8.9443473 126.26567
8.9996445 126.06417
9.0551122 125.86249
9.1107502 125.66065
9.1665587 125.45863
9.2225375 125.25643
9.2786868 125.05406
9.3350064 124.85152
9.3914965 124.6488
9.448157 124.4459
9.5049879 124.24283
9.5619892 124.03958
9.6191609 123.83616
9.676503 123.63256
9.7340155 123.42878
9.7916985 123.22482
9.8495518 123.02069
9.9075755 122.81637
9.9657697 122.61188
10.024134 122.40721
10.082669 122.20237
10.141375 121.99734
10.20025 121.79213
10.259297 121.58674
10.318513 121.38118
10.3779 121.17543
10.437458 120.96951
10.497185 120.7634
10.557084 120.55711
10.617152 120.35064
10.677391 120.14399
10.737801 119.93716
10.798381 119.73015
10.859131 119.52295
10.920052 119.31557
10.981143 119.10802
11.042404 118.90027
11.103836 118.69235
11.165438 118.48425
11.227211 118.27596
11.289154 118.06749
11.351268 117.85883
11.413552 117.65
11.476006 117.44098
11.538631 117.23177
11.601426 117.02239
11.664391 116.81282
11.727527 116.60306
11.790834 116.39313
11.85431 116.18301
11.917958 115.9727
11.981775 115.76222
12.045763 115.55155
12.109922 115.34069
12.174251 115.12965
12.23875 114.91843
12.303419 114.70703
12.368259 114.49544
12.43327 114.28366
12.498451 114.0717
12.563802 113.85956
12.629324 113.64724
12.695016 113.43473
12.760878 113.22204
12.826911 113.00916
12.893114 112.7961
12.959488 112.58286
13.026032 112.36943
13.092747 112.15582
13.159632 111.94203
13.226687 111.72805
13.293913 111.5139
13.361309 111.29955
13.428876 111.08503
13.496612 110.87032
13.56452 110.65543
13.632598 110.44035
&
@target G0.S1
@type xy
8.5203735e-05 0.0026582438
0.00034081494 0.022400569
0.00076683362 0.082980547
0.0013632598 0.22782175
0.0021300934 0.55860764
0.0030673345 1.4031316
0.004174983 4.7951315
0.0054530391 159.47857
0.0069015026 174.48586
0.0085203735 176.04438
0.010309652 176.55317
0.012269338 176.75317
0.014399431 176.82042
0.016699932 176.81829
0.01917084 176.77521
0.021812156 176.70586
0.02462388 176.61861
0.02760601 176.51856
0.030758548 176.40903
0.034081494 176.29227
0.037574847 176.16984
0.041238608 176.04288
0.045072776 175.91226
0.049077352 175.77859
0.053252335 175.64239
0.057597725 175.50404
0.062113523 175.36386
0.066799728 175.22209
0.071656341 175.07895
0.076683362 174.9346
0.08188079 174.78919
0.087248625 174.64283
0.092786868 174.49563
0.098495518 174.34767
0.10437458 174.19903
0.11042404 174.04976
0.11664391 173.89993
0.12303419 173.74959
0.12959488 173.59877
0.13632598 173.44752
0.14322748 173.29586
0.15029939 173.14383
0.15754171 172.99145
0.16495443 172.83874
0.17253756 172.68573
0.1802911 172.53244
0.18821505 172.37887
0.19630941 172.22506
0.20457417 172.071
0.21300934 171.91671
0.22161492 171.76221
0.2303909 171.6075
0.23933729 171.4526
0.24845409 171.2975
0.2577413 171.14223
0.26719891 170.98678
0.27682694 170.83117
0.28662537 170.67539
0.2965942 170.51945
0.30673345 170.36337
0.3170431 170.20714
0.32752316 170.05077
0.33817363 169.89425
0.3489945 169.73761
0.35998578 169.58083
0.37114747 169.42392
0.38247957 169.26689
0.39398207 169.10973
0.40565498 168.95245
0.4174983 168.79505
0.42951203 168.63754
0.44169616 168.47991
0.45405071 168.32216
0.46657565 168.16431
0.47927101 168.00634
0.49213678 167.84826
0.50517295 167.69008
0.51837953 167.53179
0.53175651 167.37339
0.54530391 167.21488
0.55902171 167.05627
0.57290992 166.89756
0.58696853 166.73874
0.60119756 166.57982
0.61559699 166.4208
0.63016683 166.26168
0.64490707 166.10245
0.65981773 165.94312
0.67489879 165.78369
0.69015026 165.62416
0.70557213 165.46453
0.72116442 165.3048
0.73692711 165.14497
0.75286021 164.98503
0.76896371 164.825
0.78523762 164.66487
0.80168195 164.50463
0.81829667 164.3443
0.83508181 164.18386
0.85203735 164.02333
0.8691633 163.86269
0.88645966 163.70195
0.90392643 163.54111
0.9215636 163.38017
0.93937118 163.21912
0.95734917 163.05798
0.97549757 162.89673
0.99381637 162.73537
1.0123056 162.57392
1.0309652 162.41236
1.0497952 162.2507
1.0687957 162.08893
1.0879665 161.92706
1.1073077 161.76509
1.1268194 161.60301
1.1465015 161.44082
1.1663539 161.27853
1.1863768 161.11613
1.2065701 160.95362
1.2269338 160.79101
1.2474679 160.62829
1.2681724 160.46546
1.2890473 160.30252
1.3100926 160.13947
1.3313084 159.97631
1.3526945 159.81304
1.374251 159.64966
1.395978 159.48617
1.4178754 159.32257
1.4399431 159.15885
1.4621813 158.99503
1.4845899 158.83108
1.5071689 158.66703
1.5299183 158.50286
1.5528381 158.33857
1.5759283 158.17417
1.5991889 158.00966
1.6226199 157.84502
1.6462214 157.68027
1.6699932 157.5154
1.6939355 157.35041
1.7180481 157.18531
1.7423312 157.02008
1.7667847 156.85474
1.7914085 156.68927
1.8162028 156.52368
1.8411675 156.35797
1.8663026 156.19214
1.8916081 156.02619
1.917084 155.86011
1.9427304 155.6939
1.9685471 155.52758
1.9945342 155.36112
2.0206918 155.19454
2.0470197 155.02784
2.0735181 154.861
2.1001869 154.69404
2.127026 154.52696
2.1540356 154.35974
2.1812156 154.19239
2.208566 154.02491
2.2360868 153.8573
2.263778 153.68956
2.2916397 153.52169
2.3196717 153.35369
2.3478741 153.18555
2.376247 153.01728
2.4047902 152.84888
2.4335039 152.68034
2.462388 152.51166
2.4914424 152.34285
2.5206673 152.1739
2.5500626 152.00482
2.5796283 151.83559
2.6093644 151.66623
2.6392709 151.49673
2.6693478 151.32709
2.6995951 151.15731
2.7300129 150.98739
2.760601 150.81733
2.7913596 150.64712
2.8222885 150.47678
2.8533879 150.30629
2.8846577 150.13565
2.9160978 149.96487
2.9477084 149.79395
2.9794894 149.62288
3.0114408 149.45167
3.0435626 149.28031
3.0758548 149.1088
3.1083175 148.93714
3.1409505 148.76534
3.1737539 148.59338
3.2067278 148.42128
3.239872 148.24903
3.2731867 148.07662
3.3066718 147.90407
3.3403272 147.73136
3.3741531 147.5585
3.4081494 147.38549
3.4423161 147.21233
3.4766532 147.03901
3.5111607 146.86553
3.5458386 146.6919
3.580687 146.51812
3.6157057 146.34418
3.6508949 146.17008
3.6862544 145.99583
3.7217844 145.82141
3.7574847 145.64684
3.7933555 145.47211
3.8293967 145.29722
3.8656083 145.12217
3.9019903 144.94696
3.9385427 144.77159
3.9752655 144.59606
4.0121587 144.42036
4.0492223 144.2445
4.0864563 144.06848
4.1238608 143.8923
4.1614356 143.71595
4.1991809 143.53944
4.2370966 143.36276
4.2751826 143.18591
4.3134391 143.0089
4.351866 142.83172
4.3904633 142.65438
4.429231 142.47686
4.4681691 142.29918
4.5072776 142.12133
4.5465565 141.94331
4.5860058 141.76512
4.6256256 141.58676
4.6654157 141.40823
4.7053763 141.22953
4.7455072 141.05066
4.7858086 140.87161
4.8262804 140.6924
4.8669226 140.513
4.9077352 140.33344
4.9487182 140.1537
4.9898716 139.97379
5.0311954 139.7937
5.0726896 139.61343
5.1143542 139.43299
5.1561892 139.25238
5.1981947 139.07158
5.2403705 138.89061
5.2827168 138.70946
5.3252335 138.52814
5.3679205 138.34663
5.410778 138.16495
5.4538059 137.98308
5.4970042 137.80104
5.5403729 137.61882
5.583912 137.43641
5.6276215 137.25383
5.6715014 137.07106
5.7155518 136.88811
5.7597725 136.70498
5.8041637 136.52166
5.8487252 136.33816
5.8934572 136.15448
5.9383595 135.97062
5.9834323 135.78657
6.0286755 135.60233
6.0740891 135.41791
6.1196731 135.23331
6.1654275 135.04851
6.2113523 134.86354
6.2574475 134.67837
6.3037132 134.49302
6.3501492 134.30748
6.3967556 134.12175
6.4435325 133.93584
6.4904797 133.74973
6.5375974 133.56344
6.5848855 133.37696
6.632344 133.19029
6.6799728 133.00342
6.7277721 132.81637
6.7757418 132.62913
6.823882 132.4417
6.8721925 132.25407
6.9206734 132.06625
6.9693247 131.87825
7.0181465 131.69005
7.0671386 131.50165
7.1163012 131.31307
7.1656341 131.12429
7.2151375 130.93532
7.2648113 130.74615
7.3146555 130.55679
7.3646701 130.36723
7.4148551 130.17748
7.4652105 129.98754
7.5157363 129.7974
7.5664325 129.60707
7.6172991 129.41654
7.6683362 129.22581
7.7195436 129.03489
7.7709215 128.84377
7.8224697 128.65245
7.8741884 128.46094
7.9260775 128.26923
7.978137 128.07732
8.0303668 127.88521
8.0827671 127.69291
8.1353379 127.50041
8.188079 127.30771
8.2409905 127.11481
8.2940724 126.92171
8.3473247 126.72841
8.4007475 126.53492
8.4543406 126.34122
8.5081042 126.14733
8.5620382 125.95323
8.6161425 125.75894
8.6704173 125.56444
8.7248625 125.36974
8.7794781 125.17485
8.8342641 124.97975
8.8892205 124.78445
8.9443473 124.58895
8.9996445 124.39325
9.0551122 124.19735
9.1107502 124.00124
9.1665587 123.80494
9.2225375 123.60843
9.2786868 123.41172
9.3350064 123.21481
9.3914965 123.01769
9.448157 122.82038
9.5049879 122.62286
9.5619892 122.42514
9.6191609 122.22721
9.676503 122.02909
9.7340155 121.83076
9.7916985 121.63222
9.8495518 121.43349
9.9075755 121.23455
9.9657697 121.0354
10.024134 120.83606
10.082669 120.63651
10.141375 120.43676
10.20025 120.2368
10.259297 120.03664
10.318513 119.83627
10.3779 119.63571
10.437458 119.43494
10.497185 119.23396
10.557084 119.03278
10.617152 118.8314
10.677391 118.62981
10.737801 118.42802
10.798381 118.22603
10.859131 118.02383
10.920052 117.82143
10.981143 117.61882
11.042404 117.41601
11.103836 117.213
11.165438 117.00978
11.227211 116.80636
11.289154 116.60273
11.351268 116.39891
11.413552 116.19487
11.476006 115.99064
11.538631 115.7862
11.601426 115.58155
11.664391 115.37671
11.727527 115.17166
11.790834 114.96641
11.85431 114.76095
11.917958 114.55529
11.981775 114.34943
12.045763 114.14336
12.109922 113.9371
12.174251 113.73062
12.23875 113.52395
12.303419 113.31708
12.368259 113.11
12.43327 112.90272
12.498451 112.69524
12.563802 112.48755
12.629324 112.27967
12.695016 112.07158
12.760878 111.86329
12.826911 111.6548
12.893114 111.44611
12.959488 111.23722
13.026032 111.02812
13.092747 110.81883
13.159632 110.60934
13.226687 110.39964
13.293913 110.18975
13.361309 109.97966
13.428876 109.76936
13.496612 109.55887
13.56452 109.34818
13.632598 109.13729
&
@target G0.S2
@type xy
8.5203733e-05 179.99992
0.00034081493 179.99934
0.0007668336 179.99777
0.0013632597 179.99474
0.0021300933 179.98976
0.0030673344 179.98239
0.0041749829 179.97217
0.0054530389 179.9587
0.0069015024 179.94159
0.0085203733 179.92046
0.010309652 179.89498
0.012269338 179.86484
0.014399431 179.82976
0.016699932 179.78952
0.01917084 179.74388
0.021812156 179.69269
0.024623879 179.6358
0.027606009 179.5731
0.030758548 179.50451
0.034081493 179.42998
0.037574846 179.34951
0.041238607 179.2631
0.045072775 179.17079
0.04907735 179.07264
0.053252333 178.96874
0.057597724 178.8592
0.062113521 178.74414
0.066799727 178.6237
0.071656339 178.49803
0.07668336 178.36731
0.081880787 178.23172
0.087248623 178.09144
0.092786865 177.94666
0.098495515 177.79759
0.10437457 177.64443
0.11042404 177.48739
0.11664391 177.32667
0.12303419 177.16247
0.12959488 176.99501
0.13632597 176.82449
0.14322748 176.65109
0.15029939 176.47502
0.1575417 176.29647
0.16495443 176.11561
0.17253756 175.93264
0.1802911 175.74771
0.18821505 175.561
0.1963094 175.37266
0.20457416 175.18285
0.21300933 174.99171
0.22161491 174.79938
0.23039089 174.60598
0.23933729 174.41165
0.24845409 174.2165
0.25774129 174.02063
0.26719891 173.82416
0.27682693 173.62717
0.28662536 173.42977
0.29659419 173.23203
0.30673344 173.03403
0.31704309 172.83585
0.32752315 172.63756
0.33817362 172.43921
0.34899449 172.24086
0.35998577 172.04257
0.37114746 171.84439
0.38247956 171.64636
0.39398206 171.44852
0.40565497 171.25091
0.41749829 171.05356
0.42951202 170.8565
0.44169615 170.65976
0.45405069 170.46336
0.46657564 170.26733
0.479271 170.07167
0.49213676 169.87642
0.50517293 169.68158
0.51837951 169.48716
0.5317565 169.29317
0.54530389 169.09963
0.55902169 168.90653
0.5729099 168.71389
0.58696852 168.52171
0.60119754 168.32999
0.61559697 168.13873
0.63016681 167.94793
0.64490706 167.75759
0.65981771 167.56771
0.67489877 167.37829
0.69015024 167.18932
0.70557211 167.00081
0.7211644 166.81273
0.73692709 166.6251
0.75286018 166.4379
0.76896369 166.25113
0.7852376 166.06478
0.80168192 165.87884
0.81829665 165.69332
0.83508179 165.50819
0.85203733 165.32346
0.86916328 165.13911
0.88645964 164.95514
0.9039264 164.77154
0.92156358 164.5883
0.93937116 164.40542
0.95734914 164.22288
0.97549754 164.04068
0.99381634 163.8588
1.0123056 163.67724
1.0309652 163.496
1.0497952 163.31506
1.0687956 163.13441
1.0879665 162.95406
1.1073077 162.77397
1.1268194 162.59416
1.1465014 162.41462
1.1663539 162.23532
1.1863768 162.05627
1.2065701 161.87747
1.2269338 161.69889
1.2474679 161.52053
1.2681724 161.34239
1.2890473 161.16446
1.3100926 160.98673
1.3313083 160.80919
1.3526945 160.63184
1.374251 160.45467
1.395978 160.27767
1.4178753 160.10084
1.4399431 159.92416
1.4621813 159.74764
1.4845898 159.57126
1.5071688 159.39503
1.5299182 159.21893
1.552838 159.04295
1.5759282 158.8671
1.5991889 158.69136
1.6226199 158.51573
1.6462213 158.34021
1.6699932 158.16479
1.6939354 157.98946
1.7180481 157.81421
1.7423311 157.63905
1.7667846 157.46397
1.7914085 157.28896
1.8162028 157.11402
1.8411675 156.93914
1.8663026 156.76432
1.8916081 156.58955
1.917084 156.41483
1.9427303 156.24016
1.968547 156.06553
1.9945342 155.89093
2.0206917 155.71636
2.0470197 155.54182
2.073518 155.36731
2.1001868 155.19281
2.127026 155.01833
2.1540356 154.84387
2.1812156 154.66941
2.208566 154.49495
2.2360868 154.3205
2.263778 154.14604
2.2916396 153.97158
2.3196716 153.79711
2.3478741 153.62262
2.3762469 153.44812
2.4047902 153.27361
2.4335038 153.09907
2.4623879 152.9245
2.4914424 152.74991
2.5206672 152.57528
2.5500625 152.40062
2.5796282 152.22593
2.6093643 152.05119
2.6392708 151.87642
2.6693478 151.70159
2.6995951 151.52673
2.7300128 151.35181
2.7606009 151.17683
2.7913595 151.00181
2.8222885 150.82672
2.8533878 150.65158
2.8846576 150.47637
2.9160978 150.3011
2.9477083 150.12577
2.9794893 149.95036
3.0114407 149.77488
3.0435625 149.59933
3.0758548 149.42371
3.1083174 149.248
3.1409504 149.07222
3.1737539 148.89636
3.2067277 148.72041
3.2398719 148.54438
3.2731866 148.36826
3.3066717 148.19205
3.3403271 148.01575
3.374153 147.83936
3.4081493 147.66287
3.442316 147.48629
3.4766531 147.30961
3.5111606 147.13283
3.5458386 146.95595
3.5806869 146.77897
3.6157056 146.60188
3.6508948 146.42469
3.6862543 146.24739
3.7217843 146.06998
3.7574846 145.89245
3.7933554 145.71482
3.8293966 145.53708
3.8656082 145.35922
3.9019902 145.18124
3.9385426 145.00314
3.9752654 144.82493
4.0121586 144.6466
4.0492222 144.46814
4.0864562 144.28956
4.1238607 144.11086
4.1614355 143.93203
4.1991808 143.75308
4.2370964 143.57399
4.2751825 143.39478
4.313439 143.21544
4.3518659 143.03596
4.3904632 142.85636
4.4292309 142.67662
4.468169 142.49674
4.5072775 142.31673
4.5465564 142.13658
4.5860057 141.95629
4.6256255 141.77587
4.6654156 141.5953
4.7053762 141.41459
4.7455071 141.23374
4.7858085 141.05275
4.8262803 140.87161
4.8669224 140.69032
4.907735 140.50889
4.948718 140.32731
4.9898714 140.14559
5.0311952 139.96371
5.0726894 139.78169
5.1143541 139.59951
5.1561891 139.41718
5.1981945 139.2347
5.2403704 139.05206
5.2827167 138.86928
5.3252333 138.68633
5.3679204 138.50323
5.4107779 138.31997
5.4538057 138.13656
5.497004 137.95298
5.5403727 137.76925
5.5839118 137.58535
5.6276214 137.4013
5.6715013 137.21708
5.7155516 137.0327
5.7597724 136.84816
5.8041635 136.66345
5.848725 136.47858
5.893457 136.29354
5.9383594 136.10834
5.9834322 135.92297
6.0286753 135.73744
6.0740889 135.55173
6.1196729 135.36586
6.1654273 135.17981
6.2113521 134.9936
6.2574474 134.80722
6.303713 134.62066
6.350149 134.43393
6.3967555 134.24704
6.4435323 134.05996
6.4904796 133.87272
6.5375972 133.68529
6.5848853 133.4977
6.6323438 133.30993
6.6799727 133.12198
6.727772 132.93385
6.7757417 132.74555
6.8238818 132.55707
6.8721923 132.36841
6.9206732 132.17958
6.9693245 131.99056
7.0181463 131.80137
7.0671384 131.61199
7.116301 131.42243
7.1656339 131.23269
7.2151373 131.04277
7.2648111 130.85267
7.3146553 130.66239
7.3646699 130.47192
7.4148549 130.28127
7.4652103 130.09043
7.5157361 129.89941
7.5664323 129.7082
7.6172989 129.51681
7.668336 129.32523
7.7195434 129.13347
7.7709213 128.94152
7.8224695 128.74938
7.8741882 128.55706
7.9260773 128.36455
7.9781367 128.17184
8.0303666 127.97896
8.0827669 127.78588
8.1353376 127.59261
8.1880787 127.39915
8.2409903 127.2055
8.2940722 127.01167
8.3473245 126.81764
8.4007473 126.62342
8.4543404 126.42901
8.508104 126.2344
8.5620379 126.03961
8.6161423 125.84462
8.6704171 125.64944
8.7248623 125.45407
8.7794779 125.25851
8.8342639 125.06275
8.8892203 124.86679
8.9443471 124.67065
8.9996443 124.47431
9.0551119 124.27777
9.11075 124.08104
9.1665584 123.88411
9.2225373 123.68699
9.2786865 123.48968
9.3350062 123.29217
9.3914963 123.09446
9.4481567 122.89655
9.5049876 122.69846
9.5619889 122.50016
9.6191606 122.30167
9.6765028 122.10298
9.7340153 121.90409
9.7916982 121.705
9.8495515 121.50572
9.9075753 121.30624
9.9657694 121.10657
10.024134 120.90669
10.082669 120.70662
10.141374 120.50635
10.20025 120.30588
10.259296 120.10521
10.318513 119.90435
10.3779 119.70328
10.437457 119.50202
10.497185 119.30055
10.557083 119.09889
10.617152 118.89703
10.677391 118.69497
10.7378 118.49272
10.79838 118.29026
10.859131 118.0876
10.920051 117.88474
10.981142 117.68169
11.042404 117.47843
11.103836 117.27498
11.165438 117.07133
11.227211 116.86747
11.289154 116.66342
11.351267 116.45917
11.413551 116.25471
11.476006 116.05006
11.53863 115.84521
11.601425 115.64016
11.664391 115.43491
11.727527 115.22946
11.790833 115.02381
11.85431 114.81796
11.917957 114.61191
11.981775 114.40566
12.045763 114.19921
12.109921 113.99257
12.17425 113.78572
12.238749 113.57868
12.303419 113.37143
12.368259 113.16399
12.43327 112.95635
12.49845 112.74851
12.563802 112.54047
12.629323 112.33223
12.695015 112.1238
12.760878 111.91516
12.826911 111.70633
12.893114 111.4973
12.959488 111.28807
13.026032 111.07865
13.092746 110.86902
13.159631 110.6592
13.226687 110.44919
13.293912 110.23897
13.361309 110.02856
13.428875 109.81795
13.496612 109.60715
13.564519 109.39614
13.632597 109.18495
&

